LLM-Powered Analysis of IoT User Reviews: Tracking and Ranking Security and Privacy Concerns

Being able to understand the security and privacy (S&P) concerns of IoT users brings benefits to both developers and users. To learn about users' views, we examine Amazon IoT reviews - one of the biggest IoT markets. This work presents a state-of-the-art methodology to identify and categorize reviews in which users express S&P concerns. We developed an automated pipeline by fine-tuning GPT-3.5-Turbo to build two models: the Classifier-Rationalizer-Categorizer and the Thematic Mapper. By leveraging dynamic few-shot prompting and the model's large context size, our pipeline achieved over 97% precision and recall, significantly outperforming keyword-based and classical ML methods. We applied our pipeline to 91K Amazon reviews about fitness trackers, smart speakers and cameras, over multiple years. We found that on average 5% contained S&P concerns, while security camera exhibited the highest prevalence at 10%. Our method detected significantly more S&P-relevant reviews than prior works: 15x more for fitness trackers, 29% more for smart speakers, and 70% more for cameras. Our longitudinal analysis reveals that concerns like surveillance and data control have persisted for years, suggesting limited industry progress. We demonstrate that across all device types, users consistently demand more precise control over what data is collected and shared. We uncover challenges in multi-user and multi-device interactions, identifying two previously unreported themes concerning inadequate controls for account separation and data access. These findings, ranging from broad persistent trends to specific instances of customer loss, offer actionable insights for developers to improve user satisfaction and trust.

==> Section/CRC.tex <==
\paragraphb{Candidate Reviews for Training and Validation.}
Figure \ref{CRC}, Steps 1-3 outlines the process. We collect negatively labeled (no S\&P concerns) data from the OSF Repository and manually label 600 reviews from dataset $\mathcal{W}$ as negative (Steps 1 and 2). Then, we combine them with positively labeled (S\&P concerns) reviews from the OSF Repository (Step 2), resulting in 2454 reviews, equally divided between positive and negative labels (Step 3).


\paragraphb{Objective and Task-set Specification of the Model.} Given a text $t$, the CRC model should classify if $t$ has concerns, rationalize the reason, and categorize any S\&P concerns into low-level themes. This is defined by three tasks: \textit{Task 1: Determine if $t$ explicitly mentions any security or privacy concerns. Respond only with a Yes or a No.}, \textit{Task 2: Provide a brief explanation as to why your response is as such for Task 1.}, and \textit{Task 3: If the response for Task 1 was a Yes, categorize the explicit concerns mentioned in $t$ with themes related to security and privacy}.

\paragraphb{Prompt Engineering.} Figure \ref{CRC} Step 4 outlines the prompt engineering process which incorporates two \textit{helpful examples} in the prompt. These examples include text + label for two texts, $t_{1}$ and $t_{2}$, each representing opposing labels for Task 1 (e.g., if $t_{1}$'s Task 1 label is ``Yes," then $t_{2}$'s label is ``No," and vice versa). We define two key properties for these helpful examples: idealness and affinity. Idealness ensures that the example ($t_{1}$ and $t_{2}$) is a text with an ideal label for all three tasks, typically sourced from the OSF repository's human-curated data. Affinity ensures that the examples ($t_{1}$ and $t_{2}$) are similar in context to the text $t$ under classification. This was achieved by computing BERT-embeddings and finding cosine similarities between $t$ and the rest of the texts from the training dataset. This approach enables us to provide \textit{helpful examples}, $t_{1}$ and $t_{2}$, for classifying the text $t$, enhancing the quality and relevance of our fine-tuning process. Appendix \ref{algo1} contains the algorithm that we use to generate two helpful examples $t_{1}$ and $t_{2}$ from the training dataset with their ideal labels, i.e., Task-set responses. Appendix \ref{crctemplate} shows the Prompt engineering template, and \ref{crctemplateexample} shows an actual example passed as test data from the dataset $\mathcal{W}$.

\paragraphb{Training the model and determining optimal temperature.} We perform an 80-20 split (i.e., training: 1964 reviews, validation: 490 reviews) of the candidate training and validation reviews to create the training and validation dataset for the CRC model. We then train the model using the 80\% split via the OpenAI API, which took approximately an hour to complete. Additionally, to test the performance on the 20\% split, we modulate the temperature parameter from $t=0$ to $t=0.8$ in increments of $t=0.2$ to find the optimal temperature for the model's classification rate. We find that $t=0$ yielded the best accuracy: 97.8\%  (Class 0 precision: 98\%, recall: 97.6\%, F1-score: 97.6\% and  Class 1 precision 97.6\%, recall: 98\%, F1-score: 97.8\%; see Appendix \ref{validationreport} for more details).

\paragraphb{Evaluating the performance on a subset of the wild dataset.} We randomly sample 300 reviews from the wild dataset $\mathcal{W}$, with 100 from each category, and manually annotate them to verify the model's labels. The model achieves 99\% accuracy (Class 0 precision: 99.7\%, recall: 99.3\%, F1-score: 99.5\% and Class 1 precision 77.8\, recall: 87.5\%, F1-score: 82.4\%). The confusion matrix shows 290 true negatives, 2 false positives, 1 false negative, and 7 true positives, indicating high accuracy and reliability in classifying S\&P concerns (Appendix \ref{testreport}).

\paragraphb{Passing the entire Wild dataset to the model.} Next, we pass the whole wild dataset $\mathcal{W}$ to the model. It takes around 30 hours for all the prompts to be passed to the OpenAI's API and we obtain labels for 91,149 where almost all of them generated responses in the required format except for 122, where we noticed some anomalies in the response. We discuss the anomalies in \S\ref{anomalies}.


==> Section/NewMethodology.tex <==
\section{Methodology}


\paragraphb{Data Collection.}
Figure \ref{datacollection} shows the data collection steps. First, we go to \texttt{amazon.com} (Step 1) and search for device categories like ``fitness trackers", ``smart home speakers", and ``security cameras" (Step 2). We list products and their ASINs from the first search page (Steps 3 and 4). Then, on May 15, 2023, with a crawler created with \texttt{selenium} and \texttt{BeautifulSoup}, we collect reviews for products that showed up on the first page of search results (Step 5). Finally, we structure the raw crawled data into the Wild review dataset $\mathcal{W}$ (Step 6) that we describe next. 


\paragraphb{The Wild Review Dataset $\mathcal{W}$.}
The raw crawled data from Amazon is preprocessed to obtain the Wild review dataset $\mathcal{W}$. Preprocessing includes removing empty, duplicate, and non-English reviews, resulting in 91,749 reviews (FT: 24,046; SHS: 32,179; SSCS: 35,524). These reviews are from products from 75 vendors (FT: 23; SHS: 24; SSCS: 28), identified by ASINs (Appendix \ref{products}). Although we searched on \texttt{amazon.com}, 4.02\% of reviews comes from the rest of the world (Appendix \ref{countryw}). Next, we describe the qualitative data that we used as training data for the models. 

\begin{figure*}[!t]
\centering
\includegraphics[width=1.0\textwidth]{Figure/datacollection.pdf}
\caption{The data collection process of the Wild dataset $\mathcal{W}$}
\label{datacollection}
\end{figure*}

\paragraphb{The Qualitative Data.} The qualitative data from Protick et al. \cite{protick2024unveiling} works as training data to fine-tune our models.
This dataset is derived from a three-step processing of IoT product reviews: keyword selection, review labeling, and thematic analysis, all performed by multiple coders with reported high inter-rater reliability. This dataset is used to train our Classifier-Rationalizer-Categorizer (CRC) model and Theme Mapper (TM) model. The authors made their labeled datasets public in an OSF repository. \footnote{The repository is available here\url{https://osf.io/x4npj/?view_only=dd37575bf1d9414c9e463fd1dd5cadaf}}


\paragraphb{Selection of The Large Language Model.}
We choose \texttt{gpt-3.5-turbo} to fine-tune the CRC and TM models. On September 3, 2023, we obtained a key from OpenAI when \texttt{gpt-3.5-turbo} was the most advanced model allowing fine-tuning with proprietary API keys. We use this model for several reasons. Firstly, it has the highest token and batch queue limits among all models on \texttt{platform.openai.com}, allowing up to 1 million tokens per minute and 100 million tokens per day for Tier 4 users (as of June 1, 2024) \cite{ratelimit}, providing flexibility for fast training with large prompts. This information finds support from Ye et al. \cite{ye2023comprehensive}, who argue that it is the most capable among the \texttt{gpt-3.5-series} models (\texttt{code-davinci-002}, \texttt{text-davinci-002}, \texttt{text-davinci-003}, and \texttt{gpt-3.5-turbo}) and optimized for chat at one-tenth of the cost of \texttt{text-davinci}. Secondly, we see the recent use of \texttt{gpt-3.5-turbo} in several domains related to information retrieval such as understanding of ultrasound medical reports \cite{wang2024investigation}, combinatorial problem solving \cite{masoud2024exploring}, and extracting information from scientific articles on diabetic retinopathy \cite{gue2024evaluating}. Finally, its performance compared to other models finds support in the work of Addlesee et al. \cite{addlesee2023multi}. The study finds that while multi-party conversations remain challenging for state-of-the-art LLMs, GPT-3.5-turbo significantly outperformed T5 in few-shot settings, achieving higher accuracy in goal tracking and intent-slot recognition tasks with limited data.

\subsection{The Classifier-Rationalizer-Categorizer (CRC) Model}
\begin{figure*}[!t]
\centering
\includegraphics[width=1.0\textwidth]{Figure/CRC_qual.pdf}
\caption{The fine-tuning process for the CRC model}
\label{CRC}
\end{figure*}
\input{Section/CRC}


\paragraphb{The Theme Mapper (TM) Model.}\label{thetmmodel}
\begin{figure*}[!t]
\centering
\includegraphics[width=1.0\textwidth]{Figure/TM_qual.pdf}
\caption{The fine-tuning process for the TM model}
\label{TM}
\end{figure*}
\input{Section/TM}


\subsection{Data Analysis}
\paragraph{Statistical tests.}
The CRC model classifies 4,896/91,149 reviews with S\&P concerns. To examine if S\&P concerns vary across FT, SHS, and SSCS categories, we define the \textit{concern ratio} for $c$ as $|C_{c}|/|R_{c}|$, where $|C_{c}|$ is the number of reviews with S\&P concerns and $|R_{c}|$ is the total number of reviews for category $c$. We use the Chi-squared test for proportions (R package: \texttt{prop.test} \cite{proptest}). If the null hypothesis is rejected, we identify which pairs' concern ratios differ significantly. For multiple comparisons, we apply Bonferroni correction \cite{bonferronicorrection} to control the familywise error rate. We then test for a correlation between S\&P concerns and user ratings using a point-biserial correlation test \cite{pbs}, as S\&P concerns are dichotomous and ratings are ordinal. We interpret the correlation coefficient from \cite{kuckartz2013statistik}. Finally, we run a two-sample $t$-test \cite{ttest} between the average ratings of concern and non-concern reviews. Since the formula used to compute the test statistic of the $t$-test depends on the homogeneity of variance of the parameter, we first conduct Levene's test \cite{levtest} for homogeneity in variance in the ratings.

\paragraph{Discussion of the high-level themes based on topics.}
We partitioned the 85 high-level themes further into 11 topics and discuss them qualitatively with user reviews from each topic in \S\ref{thetmmodeltopics}. 

==> Section/Results.tex <==
\section{Results}

% The CRC model classifies 4,896/91,149 reviews with S\&P concerns. To examine if S\&P concerns vary across FT, SHS, and SSCS categories, we define the \textit{concern ratio} for a device category, $c$ as $|C_{c}|/|R_{c}|$, where $|C_{c}|$ is the number of reviews with S\&P concerns and $|R_{c}|$ is the total number of reviews for category $c$. We use the Chi-squared test for proportions \cite{proptest}. If the null hypothesis is rejected, we identify which pairs' concern ratios differ significantly. For multiple comparisons, we apply Bonferroni correction \cite{bonferronicorrection} to control the family-wise error rate. We then test for a correlation between S\&P concerns and user ratings using a point-biserial correlation test \cite{pbs}, as S\&P concerns are dichotomous and ratings are ordinal. 
% We interpret the correlation coefficient \cite{kuckartz2013statistik} to infer correlations. Finally, we run a two-sample $t$-test \cite{ttest} between the average ratings of concern and non-concern reviews. Since the formula used to compute the test statistic of the $t$-test depends on the homogeneity of variance of the parameter, we first conduct Levene's test \cite{levtest} for homogeneity in variance in the ratings.


%Below are the results.
\subsection{RQ1}\label{rq12}
% \begin{figure}[!t]
% \centering
% \includegraphics[width=0.4\textwidth]{Figure/pieconcerns.pdf}
% \caption{The part-to-whole ratio of concerned reviews across three device categories.}
% \label{pieconcerns}
% \end{figure}
\begin{figure}[!t]
\centering
\includegraphics[width=0.5\textwidth]{Figure/stackedconcerns.pdf}
\caption{The part-to-whole ratio of concerned reviews across three device categories.}
\label{pieconcerns}
\end{figure}
The CRC model detected 4,896/91,149 (5.37\%) reviews to have S\&P concerns. In this section, we conduct a couple of statistical tests. Firstly, we conduct a test to see if the concern ratio varies across product types. Next, we run a correlation test between the S\&P concerns and ratings given in a review to see the relationship between these two variables. Finally, we run a two-sample $t$-test to see if the average ratings of reviews with S\&P concerns differ significantly from that of the ones with no S\&P concerns.
\input{Table/chisq}
\input{Table/levtest}
\input{Table/ttest}

\subsubsection{Independence of concern ratio across categories of products.}
The chi-squared test for proportion (Table \ref{chisquaredtable}, middle) assesses whether the concern ratio is consistent across the product categories FT, SHS, and SSCS. The concern ratios were 0.0211 for FT, 0.0264 for SHS, and 0.1007 for SSCS. The test yielded a $p$-value of less than $2.2e-16$, indicating a highly significant difference in concern ratios across the categories. Pairwise comparisons (Table \ref{chisquaredtable}, bottom) showed significant differences between each pair of categories (FT vs. SHS: $p = 2.00e-04$, FT vs. SSCS: $p < 2e-16$, SHS vs. SSCS: $p < 2e-16$), rejecting the null hypothesis and confirming that the concern ratios are not the same across FT, SHS, and SSCS. \textit{Takeaway: SSCS has the highest concern ratio across all the device categories.}

\subsubsection{Correlation between S\&P concerns and review ratings.} We ran a point-biserial correlation test (Appendix \ref{pointbiserialtest}) between S\&P concerns and review ratings. The correlation coefficient category-wise and overall shows no correlation in SHS but low negative correlation (according to \cite{kuckartz2013statistik}) otherwise (FT: $r_{pb} = -.11$, SHS: $r_{pb} = -.06$, SSCS: $r_{pb} = -.19$, overall: $r_{pb} = -.13$). This indicates that review ratings negatively correlate to S\&P concerns, supporting Vetrivel et al. \cite{vetrivelexamining}. 

\textbf{Takeaway: S\&P concern (Label 1) is slightly negatively correlated with review ratings, i.e., Label 1 slightly implies lower stars.}


\subsubsection{Average ratings in reviews with concerns vs. reviews with no concerns.}
Next, we conduct a 2-sample $t$-test \cite{ttest} between the average ratings in the concern and non-concern reviews (Table \ref{2samplettest}). But first, we run Levene's test \cite{levtest} for homogeneity in variance between ratings of concern and non-concern reviews (Table \ref{levenetest}). This is necessary since the formula used to compute the test statistic for the $t$-test is dependent on the homogeneity in variance of the rating between the two samples. The Levene's test rejects the null hypothesis in all the cases and for which we set the \texttt{VAR.EQUAL} parameter to \texttt{FALSE} in R. The $t$-test rejects the null hypothesis that the average ratings of the concern reviews and non-concern reviews are equal. \textbf{Takeaway: Reviews with S\&P concerns have a significantly lower rating than those without S\&P concerns.}

%\input{Table/review-crc-tm}
\subsection{The TM model}\label{thetmmodeltopics}
\begin{figure*}[!t]
\centering
\includegraphics[width=1.0\textwidth]{Figure/pie-topten.pdf}
\caption{Frequency of the top ten themes per device category.}
\label{pietopten}
\end{figure*}
% commented out

%  When passed to the CRC model, all 4,896 reviews with S\&P concerns had Task 1 response as ``Yes'' and Task 3 response categorized to at least one low-level theme related to S\&P. Overall, we found 14,981 (9,720 unique) low-level themes in the Task 3 responses. Each of these Task 3 responses had been passed to the TM model so that the model could map them to one or more related high-level themes (Table \ref{revcrctm}, right column). Figure \ref{barchartcounts} shows the number of times any low-level themes were mapped to any of these 85 high-level theme(s).  The ten most frequently mapped high-level themes were: \textit{Surveillance (1894), Privacy Invasion: (1562),
% Technical and Technological Issues (1331), Usability (1325), Lack of Authentication and Authorization (1121), Access Control (1097), User Preference (721), Data Privacy (661), Data Security (655)},
% and \textit{Eavesdropping (599)}. The high-level themes least mapped to by any low-level themes were ``Access / participation", ``Appropriation", ``Being self-righteous about privacy", and ``Purpose specification" (One time). In this section, we discuss the content of the reviews under related high-level themes.

% % \begin{figure}[!tb]
% % \centering
% % \includegraphics[width=1.0\textwidth]{Figure/counts.pdf}
% % \caption{The bar-chart shows the number of times any low-level themes were mapped to a high-level theme. The high-level theme most mapped to by any low-level themes was ``Surveillance'' (1894 times). The high-level theme least mapped to by any low-level themes were ``Access / participation", ``Appropriation", ``Being self-righteous about privacy", ``Purpose specification" (One time).}
% % \label{dvalhisto}
% % \end{figure}
% \begin{figure*}[!t]
% \centering
% \includegraphics[width=1.0\textwidth]{Figure/counts.pdf}
% \caption{The bar-chart shows the number of times any low-level themes were mapped to a high-level theme.}
% \label{barchartcounts}
% \end{figure*}
%\input{Table/topics}

% \begin{figure*}[!t]
% \centering
% \includegraphics[width=1.0\textwidth]{Figure/histogram.pdf}
% \caption{Counts of concerns category-wise (subject to change).}
% \label{categorywisehistogram}
% \end{figure*}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.4\textwidth]{Figure/pi_ft.pdf}
% \caption{Pie chart showing topic-wise concerns for fitness trackers (subject to change).}
% \label{pift}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.4\textwidth]{Figure/pi_shs.pdf}
% \caption{Pie chart showing topic-wise concerns for smart home speakers  (subject to change).}
% \label{pift}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.4\textwidth]{Figure/pi_sscs.pdf}
% \caption{Pie chart showing topic-wise concerns for security cameras  (subject to change).}
% \label{pift}
% \end{figure}
% \input{Table/topics}
% \input{Table/topics}

% \subsubsection{Reviews in related high-level themes.}
% For space constraint, we restrict ourselves from discussing all the 85 themes and reviews mapped to them. Instead, we subjectively partition the high-level themes into eleven meaningful topics (Table \ref{elevenbroadtopics}). Each topic is discussed below with an example review. Since a review can be mapped to more than one high-level themes where those themes can be member of different topics, we boldfaced the high-level themes under our topic of discussion. 

% \paragraphb{Data Security (2,333 reviews).} S\&P concerns related to Data Security focus on protecting sensitive data, including personally identifiable information (PII), from unauthorized access and breaches. These concerns include secure data deletion and preventing unauthorized modifications. Robust security measures are essential to protect user data. For example, the review FT-2996 highlights data security and availability issues, where stored data disappeared, and the device failed to sync, causing a loss of two days' data. Additionally, the lack of a warning when deleting data raises privacy concerns, emphasizing the need for secure deletion practices and better user notifications. Addressing these issues is crucial for maintaining data security and user trust.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \largestar \largestar \largestar$
% \normalsize
% (FT-2996)``Stored data somehow disappeared. Device won’t sync for unknown reason. Tried all of sync options but didn’t work. The only way was to get to sync to work again was to drain the battery completely. Of course I lost two days of data. Be aware that if you edit any of your data on app, make sure you select the “edit” button. There is no warning if you accidentally hit the delete option."  $->$ [\textbf{`data availability', `data security'}, 'data privacy', \textbf{`data deletion'}, 'notice / awareness']
% \end{myquote}

% \paragraphb{Trust and Transparency (2,457 reviews).}
% Trust and Transparency are vital aspects of digital interactions, ensuring security and privacy. The review FT-27118 highlights business practice transparency and usability challenges, which are essential aspects of trust and transparency in digital interactions. The user's experience of spending over ten minutes trying to pair the device in the app, coupled with prompts for credit card information to subscribe, reflects a lack of transparency and convenience in the setup process. This scenario raises concerns about payment security and the need for clear information and user-friendly interfaces to build trust and satisfaction in digital environments.
% \begin{myquote}
% \tiny
% % $\bigstar \largestar \largestar \largestar \largestar$ 
% \normalsize
% (FT-27118) ``Spent over ten minutes trying to get it to pair in the app while getting inundated with prompts for my credit card to get a subscription. I will be returning this. It seemed like a nice feature to be able to check my temp and BP but too much of a headache to set up.
% " $->$ [`payment security', \textbf{`business practice transparency'}, `usability']
% \end{myquote}

% \paragraphb{Security Threats and Incidents (2,121 reviews).}
% Users face security challenges such as lack of authentication, concerns about eavesdropping, and breaches of confidentiality, which can lead to privacy violations and trust issues. Privacy concerns in this context involve safeguarding sensitive information from unauthorized access, ensuring confidentiality, preventing data breaches, and addressing potential risks posed by hackers and malicious actors. Mitigating these threats requires robust security measures, regular monitoring, and adherence to best data protection and privacy management practices. The review SSCS-68 exemplifies these concerns, detailing an incident where a baby monitor appeared to be hacked, leading to fears of privacy invasion and unauthorized surveillance. Despite having up-to-date software and network security measures, the user's experience with the device's suspicious behavior and potential eavesdropping highlights the critical need for stringent access control and authentication protocols to maintain trust and privacy preservation in security devices.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \largestar \largestar \largestar$
% \normalsize
% (SSCS-68)``we used this for a few weeks as a baby monitor, but then it appeared to get hacked so we stopped using it completely. while it worked, we really ... (gap) ... but then one day it started clicking on and off by itself (the lens was opening and closing and brief recordings were listed in the blink app).none of us were using the camera at the time.this was very suspicions, and having someone else looking at our child in bed is terrifying.i am quite tech savvy, and take security seriously. we have at-the-network security to help with all of the internet-of-things devices that tend to be less secure than a pc with a firewall. or just a router that has all kinds of holes and exceptions that many products automatically create..the device was up-to-date with the latest software and firmware.i normally don't write negative reviews, but thought people would want to know about the risk.i normally stay away from negative reviews, but given that people use these cameras for their homes...ultimately, if you don't care about what the camera is viewing being secure, it is a great little device."  $->$ ['surveillance', \textbf{`eavesdropping'}, `privacy invasion', `privacy preservation', `lack of trust in the device', `access control', `lack of authentication and authorization', `privacy controls']
% \end{myquote}

% \paragraphb{Privacy Controls and Preferences (2,117 reviews).} Concerns in this topic revolve around ensuring secure access and handling of data, preventing unauthorized access or misuse, and maintaining confidentiality and integrity throughout data processing activities. Privacy concerns encompass protecting individuals' privacy rights, having the ability to provide consent regarding data collection, avoiding data breaches or exposure, and upholding transparency, accountability, and ethical practices in data management. The review SHS-13044 highlights privacy concerns regarding data access and permissions for the Echo smart speaker, indicating that users must consent to extensive data collection to fully use the device. This aligns with the broader issues of secure data handling, preventing unauthorized access, and ensuring transparency and accountability in data management.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \bigstar \bigstar \largestar$ 
% \normalsize
% (SHS-13044)``...Oh, and if you’re the nervous about your info type person, Echo might not be for you! She required permissions to anything and everything in order for you to take full advantage of the fun and benefits of using this smart speaker.Should I discover any more pros or cons that I think might be helpful, I’ll add here."  $->$ [\textbf{`consent'}, `data collection']
% \end{myquote}

% \paragraphb{Monitoring (2,013 reviews).} Monitoring involves various practices like location tracking, surveillance, and activity tracking. While these methods can enhance security by enabling real-time monitoring and threat detection, they also raise significant privacy concerns. Location and tracking can infringe on individuals' privacy by recording their movements and activities. Tracking activities for analytics or personalization purposes can also compromise user privacy if not handled transparently and responsibly. The review FT-1937 highlights concerns related to data collection, location tracking, and usability in monitoring practices. The user's experience of encountering annoying warnings while syncing due to location permissions raises questions about data harvesting techniques and privacy invasion.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \bigstar \largestar \largestar$ 
% \normalsize
% (FT-1937)``... (gap) ... -App wants location, full precise location to sync. Well it gives you annoying warnings but still syncs. Assuming this is their data harvesting techniques.-Sleep score works half the time. Seems quite gimmicky and always has.-Clock faces are awful and cannot be customized."  $->$ [`data collection', \textbf{`location and tracking', `tracking'}, `selling data', `data integrity', `usability', `user preference']
% \end{myquote}

% \paragraphb{Physical and System Security, 1960 reviews}
% This topic encompasses protective measures for physical assets and digital systems, including intrusion detection, access control, and safety protocols. Users are concerned about app vulnerabilities that may lead to data leaks, unauthorized access, or malware attacks, compromising their security and privacy. For example, the review FT-9630 highlights concerns about system security, specifically regarding Wi-Fi security. The mention of the device tracking Wi-Fi and phone usage raises concerns about potential vulnerabilities and privacy risks associated with data sharing and tracking practices. These issues underscore the importance of robust security measures, including secure communication protocols and protection against unauthorized access, to safeguard user data and maintain system integrity.
% \begin{myquote}
% \tiny
% % $\bigstar \largestar \largestar \largestar \largestar$
% \normalsize
% (FT-9630)``First off the box you have to destroy to even get to the purchased item. Then the app you have to sync not only t your phone but to your email. Then it still say's you need to pair the device to blutooth which I had already done. Not only does it track yur wi-fi it tracks your phone."  $->$ [\textbf{`physical security'}, 'data sharing', 'data privacy', 'secure communication', 'tracking', \textbf{`wi-fi security'}, 'location and tracking']
% \end{myquote}

% \paragraphb{User Interaction and Usability (1,327 reviews).}
% S\&P concerns related to this topic may revolve around balancing usability with privacy protection, ensuring that user-friendly designs do not compromise the user's privacy. The review SSCS-3551 highlights these issues, as the user struggles with a security camera's motion sensitivity and privacy zone settings. Despite attempts to tweak settings and block activity zones, the user continues to receive numerous notifications, indicating that the usability of the privacy features is inadequate. This example illustrates the need to ensure that privacy controls are effective and user-friendly without compromising security or causing frustration.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \largestar \largestar \largestar$
% \normalsize
% (SSCS-3551)``I have spent days trying to tweak the right motion sensitivity settings its down to 3 ! and block out activity zones. The activity zone feature is useless it still picks up motion from every car passing and ive blocked the street off entirely including blocking off the neighbors across the streets houses to see if that would help and it didnt. I get countless of notifications of cars passing by. How about creating a activity zone feature that actually works ? Very frustrating  i even tried the privacy zone to completely block out the imagine of street and still did not work! disappointed feel like a waste of money."  $->$ [\textbf{`usability'}, `user preference', `seclusion']
% \end{myquote}

% \paragraphb{Data Handling and Processing (1,311 reviews).}
% Data Handling and Processing involves managing and processing data through various operations such as collection, storage, sharing, and dissemination. Users need robust security measures to protect their data from unauthorized access, misuse, or breaches during these processes. This includes implementing data encryption, access controls, transparency measures, and adhering to privacy policies to safeguard user privacy. Privacy concerns in this area revolve around ensuring transparency, consent, and compliance with privacy regulations during data collection, sharing, and onward transfer. Additionally, preventing data misuse, unauthorized disclosure, and unethical practices like selling data for profit are critical to addressing privacy concerns and maintaining user trust. The review FT-2881 underscores these concerns by highlighting the invasive nature of data collection practices, particularly the requirement to have location services on for syncing, which can lead to privacy invasion and surveillance. Such practices raise concerns about tracking, data misuse, and potential privacy violations, emphasizing the need for companies to prioritize user privacy and implement transparent and ethical data handling practices.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \largestar \largestar \largestar$
% \normalsize
% (FT-2881)``App requires 'location' to be ON to sync...  Invasive of privacy.Sleep function constantly breaks my sleep into small groups failing to give accurate feedback.Heart monitor reads intmtnt and AFib never detects anything but normal rhythm. Try Samsung or I-watch, they have to be better!
% "  $->$ ['location and tracking', 'tracking', 'surveillance', 'privacy invasion', \textbf{`data misuse'}]
% \end{myquote}

% \paragraphb{General Concerns (665 reviews)} This topic encompasses a range of issues, including generic privacy and security concerns, feelings of insecurity, distrust in devices, humor/sarcasm to express concerns, personal skepticism, indifference to privacy, willingness to trade privacy for utility, and self-righteous attitudes about privacy. The review SHS-2845 reflects concerns related to some of them. It includes general concerns such as generic privacy and security concerns, insecurity, and distrust in devices.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \bigstar \bigstar \bigstar$ 
% \normalsize
% (SHS-2845) ``I don't like how anybody can just play with my alexa when I'm not home always turning on and on things over and over"  $->$ [`access control', `lack of authentication and authorization', \textbf{`lack of trust in the device'}, `privacy preservation']
% \end{myquote}

% \paragraphb{Legal and Ethical Considerations (261 reviews).}
% Users' security in this context involves adherence to legal requirements, privacy standards, and ethical practices to protect data and ensure accountability. Privacy concerns may arise from government surveillance activities and the potential implications for individual privacy rights, transparency, and trust in the use of data for intelligence or control purposes. The review FT-1550 reflects these concerns, as the user expresses distrust towards a company perceived as a "creepy data hoarder" and criticizes the influence of big tech corporations on personal privacy. This highlights the importance of data integrity, adherence to privacy policies and laws, and minimizing data collection to build trust and ensure privacy protection.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \bigstar \largestar \largestar$ 
% \normalsize
% (FT-1550)``...If id realized what a proprietary company firbit is or if i could find a decent device from A vendor that was not such a creepy data hoarder i would have definitely bought elsewhere. We need to stop letting these big tech and evil corps stop running our world."  $->$ [`data integrity', `technical and technological issues', `data collection', `company's affiliation', `data minimization', \textbf{`privacy policies and laws'}]
% \end{myquote}

% \paragraphb{Fairness and Ethical Use (10 reviews).}
% This topic concerns maintaining equitable treatment and ethical practices concerning data access, protection, and decision-making. The review SSCS-14059 highlights fairness concerns regarding access control and authentication issues. Specifically, it mentions the difficulty in resetting the camera and moving it to another account without specific requirements, which can be seen as unfair treatment for users who do not meet those criteria. This situation raises questions about fairness in applying security measures and usability, especially for international users or those moving around. It underscores the importance of addressing fairness concerns to ensure equitable treatment and ethical use of technology across diverse user groups.
% \begin{myquote}
% \tiny
% % $\bigstar \bigstar \bigstar \bigstar \bigstar$ 
% \normalsize
% (SSCS-14059)``It’s basically impossible to reset camera and move to another account if you don’t have access to the same phone number AND Amazon account that the cameras were originally set for. Horrible for someone moving around - and totally useless for international users. Great for stationary Americans though so guess that’s were Amazons prioritized customers are located."  $->$ [`technical and technological issues', `system/application', `usability', `user preference', `access control', `lack of authentication and authorization', `affiliation with a country or a geographic region', \textbf{`fairness'}]
% \end{myquote}








==> Section/TM.tex <==
\paragraph{Candidate reviews for training and validation.}
Since the job of the TM model is to map a low-level S\&P theme to high-level theme(s), we use only the positively labeled training examples used to train the CRC model. We also use the positively labeled validation examples to validate and evaluate the performance of the TM model. Figure \ref{TM} Steps 1 and 2 outline the process.

\paragraph{Objective and task-set specification of the model.} Given a text $x$, the TM model should map $x$, a low-level S\&P theme to high-level S\&P theme(s).  We define one task for the model: \textit{Given $x$, a low-level theme related to security and privacy and $Y$ a list of high-level themes related to security and privacy, map $x$ to one or more $y$'s. This means map $x$ to one or more appropriate $y$'s from $Y$. Respond in the form $x->y_{1}$ if $x$ should be mapped to just one $y$. Respond in the form: $x->y_{1}, y_{2}, ..., y_{n}$, if $x$ should be mapped to more than one $y$}.

\paragraph{Collection of high-level themes and creation of the training and the validation set.} Figure \ref{TM} Step 3 outlines the process. We collect the high-level themes from prior work on IoT security taxonomies \cite{akbar2021multicriteria,das2018taxonomy,gulzar2019internet,williams2019security,chen2018internet}, privacy taxonomies \cite{sarwar2019brief,alsubaei2017security,ogonji2020survey,akil2020privacy,harkous2022hark,akgul2024decade}, and taxonomies that cover both security and privacy aspects \cite{solove2005taxonomy,wang2009privacy,alqassem2014taxonomy,alsamani2018taxonomy,rizvi2018securing}. 
We also add the OSF repository's  \cite{osf} high-level themes and derive some of the themes from our empirical observation. Empirical themes are \textit{fairness, fraud, being self-righteous about privacy, business practice transparency, recognizing privacy concerns but showing indifference},
and \textit{trading privacy for utility}. Appendix \ref{themeswithdefs} shows the high-level themes with their definitions, and Appendix \ref{themesrc} shows the themes with their source. Overall, they sum up to 85 themes. Next, from the candidate training and validation datasets, a human annotator maps each low-level theme (Task 3 response of the CRC model)  
to high-level theme(s) using the OSF repository's thematic analysis codebook so that related low-level themes are partitioned under appropriate high-level theme(s).

\paragraph{Prompt engineering.} Figure \ref{TM} Step 4 outlines the prompt engineering. The TM's prompt also has \textit{helpful examples}. They are ideal mappings coming from the training dataset for this model. We provide five examples of low-level themes ($A$, $B$, $C$, $D$, $E$) and their corresponding high-level mappings. Like the CRC model's helpful example, we preserve the idealness and affinity properties here. Affinity is ensured by showing five low-level themes closest to the theme that needs to be mapped by the model. This is achieved by computing TF-IDF embeddings and cosine similarities among the themes in the dataset. Unlike BERT, we use TF-IDF to preserve affinity for the TM model. This was done because, for short phrases, the TF-IDF embedding shows more relevant examples than the BERT embedding. This approach enables us to provide high-level examples for TM to map $x$ correctly. Appendix \ref{algo2}  contains the algorithm used to generate helpful examples with their ideal mappings. Appendix \ref{tmtemplate} shows the prompt engineering template, and Appendix \ref{tmactualexample} presents an actual example.

\paragraph{Training the model.} The comma-separated Task 3 responses from the CRC model are broken down into individual low-level themes. We obtain 1989 such themes (1200 unique). Then we create a prompt like Appendix \ref{tmactualexample} for each low-level theme and pass the training dataset to OpenAI for training. The model took two hours to be fine-tuned. Figure \ref{TM}, Steps 5-7 outlines this process.
 
\paragraph{Evaluating the performance on the validation dataset.} Figure \ref{TM}, an arrow from Step 5 to Step 7 outlines the process. Here, we break down all Task 3 responses of the validation data into individual low-level themes and pass them to the trained model, which amounts to 360 unique low-level themes. Later, a human annotator manually checks the mapping to evaluate the model's performance. A four-point scale of excellent, good, moderate, and poor mapping is used. All the moderate and poor mappings had been considered incorrect, and the excellent and good mappings had been considered correct. In this labeling, we see the TM model to perform well with 96.11\% accuracy (see Appendix \ref{tmvalidperformance} for details).

\paragraph{Passing the Task 3 responses from dataset $\mathcal{W}$.} The CRC model had the response ``Task 1: Yes" for 4,896 reviews. For these reviews, we had a total of 9,720 unique Task 3 responses. We passed them individually to the TM model for mapping.  


==> Section/apdx_camera_quotes.tex <==
\newpage
\section{Camera Reviews Requesting Granular Privacy Controls}
\label{cameraquotes}

\begin{table}[!h]
\caption{Additional reviews requesting granular privacy controls based on the recipient for the Camera device type}
\centering
\footnotesize
%\begin{tabularx}{\textwidth}{@{} XXX @{}}
\begin{tabular}{p{2.5cm}|p{14cm}}
%\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Recipient} & \textbf{Review} \\
\toprule
Roommate &
My roommate demanded to have access to the cameras but giving her access meant she had total control of them, including but not limited to deleting videos or shutting the cameras off. I do not like this at all so I had to get rid of them. When I get my own house I will absolutely buy these again. \\
\hline
Employees or Housesitters & You can't add other users to your account; for example, another employee or a housesitter. I want other people to be able to view notifications and the videos, but not necessarily change settings. Currently the only option is to give my password to other users which means that can edit everything. Again, it seems users have been asking for this feature to be added for a few years, but it hasn't been done. \\
\hline
Family (Multiple Properties) &
If you have multiple properties and /or need to share access to the cameras just on certain properties WITHOUT full access, DO NOT BUY THESE CAMERAS. Do not use [PRODUCT] at all. I have an aging mother and gave her access to view her cameras and had to give full access. And when I wanted to install cameras on my property and my rental I was told I would have to start a whole new Amazon account AND get another subscription. Then it requires me to log in and out all day to keep a consistent eye on all of the properties. \\
\hline
%Family at Multiple Properties & So a family of four would like to monitor the home of our 96-yr old mother. But [COMPANY] insists you can only setup one account, and that account requires 2-step authentication to login. So imagine if my sister wants to view the camera. She has to login with my credentials on HER phone, then I get a 6-digit code sent to MY phone, which I then have to text to HER so she can login. Did they not think this through??? This should be tied to your [COMPANY] account and then allow a list of phone numbers to be assigned to the account that can login for viewing.\\
Family & I bought 9 [BRAND] cameras over the years and they worked well and customer service was excellent. Since [COMPANY] bought [BRAND], however, they force you to connect everything to one [COMPANY] account—and you end up sharing your entire system with family members. With the old [BRAND] Cam you could share ONLY camera access. Now you must give someone full access to your entire account. Beware… \\
\hline
%Neighbor, Child, Relative, Visitor & User access cannot be customized. The only way to give someone access to a camera is to give them your password to your account and entire system. It would be helpful to be able to grant someone limited or temporary access, such as a neighbor, child, relative, or visitor. \\
%\hline
%Family and Friends & Video quality is...fine. Nominally 1080p, but about what you would expect from a cheap 2000s-era webcam. You will not be sharing clips with family and friends. \\
Police and Other Agencies & 
The lack of data/privacy is deplorable. Look up he they are letting police and other agencies get access w/o warrant or uses knowledge. \\
\hline
%Company
%& I own a bunch of these cameras but will replace them and never buy a [COMPANY] products as long as they give MY FOOTAGE to authorities without consent or warrant. Do not enable this behavior by supporting [COMPANY]. \\
%\hline
Company & NOT JUST [COMPANY] BUT, too many companies want access to way to much personal information and people really need to look at the fine print before DWNLG APPS, you may be signing your life away for all you know w/ the fine print ! Many Companies are doing this and its starting to feel like we are being controlled and told how and what to buy and watch / and what Big Business says we should. \\
\hline
Cloud &  I thought that these were just for recording for personal use. I DIDN'T know that EVERY video went to the "cloud" if I wanted EVERYONE to see what I was recording I would go public. I'm sending them back. \\
\hline
General &
Also they don't have separate accounts for each user and that poses a problem too have one account everyone uses with one set of sign ins. They can make changes to your system and that doesn't work for me. This is a very basic camera system that can be expanded but I'm not going to expand until they enhance the features. \\
\hline
General &
Multiple cameras cannot be viewed at the same time, nor can two users view the cameras simultaneously.
\\ \bottomrule
\end{tabular}
\end{table}

==> Section/apdx_themes.tex <==
\newpage
\subsection{High-level themes with their definitions}\label{themeswithdefs}
\small
\begin{enumerate}
\item \textbf{Access Control:} Access control involves managing users' access to resources provided by an IoT network or IoT device. A key attraction of IoT is its capability to enable data and service sharing between devices, which raises security concerns and underscores the importance of implementing an access control framework in IoT systems. Access control techniques are crucial system components in protecting IoT systems.
\item \textbf{Anonymity:} This refers to scenarios in which the user would prefer to remain anonymous and hide their identity. They may be fearful of their identity being exposed. It can also refer to rendering the activity of one group invisible to other groups, such as in a classroom, enterprise, or social media setting. Technologies such as VPNs can offer a degree of anonymity.
\item \textbf{Authentication:} Authentication is the process of verifying the identity of a user attempting to access a network or device. The proof of identity can be based on "something I am," "something I have," or "something I know."
\item \textbf{Authorization:} Authorization refers to the process of deciding whether an authenticated entity (a user or device) is allowed to access resources within an IoT network. The authorization process is typically managed through groups, roles, privileges, and permissions.
\item \textbf{Availability:} In the context of IoT, availability refers to ensuring that the network or device is accessible whenever the user requires it. This is particularly crucial when a device is replaced with a new one, as the new device should be able to access or retrieve historical data.
\item \textbf{Confidentiality:} Confidentiality refers to the protection of sensitive data generated, transmitted, and stored by IoT devices, ensuring that it is only accessible to authorized users or systems. It prevents interception or disclosure of information as it flows across networks, which is especially critical in IoT due to the vast number of interconnected devices and the frequent transmission of data over public or unsecured networks. Confidentiality in IoT is often achieved through mechanisms like encryption, secure communication protocols, and access control measures.
\item \textbf{Consent:} Consent refers to the user's sense that they have agreed to or authorized the collection, storage, sharing, and use (such as for personalization) of their data. Consent includes the concept of opt-out when users refuse consent for a specific type of data collection and use. It also includes the idea of forced consent, which is when users have to consent to the collection of a specific type of data simply in order to use an app or service.
\item \textbf{Data Accuracy:} Maintenance of the accuracy, consistency, and reliability of data throughout its lifecycle to prevent corruption, alteration, or unauthorized changes that could compromise trust or reliability.
\item \textbf{Data Collection:} This refers to the collection of personally identifying information (such as email, phone number, address), behavior activity data (from sensors, IoT devices and personal devices), as well as the collection of user-generated content. When this is useful for app functionality, it is considered purposeful and acceptable. When there is no direct purpose, it is viewed as unnecessary and a privacy violation. Collecting the minimal amount of personal data needed for the core functionality of a smartphone app, IoT skill, or web service is considered a privacy best practice.
\item \textbf{Data Deletion:} This usually refers to personal data that a user wants to delete. Examples include generated content such as files, photos, and videos. Other examples include behavior history such as cookies, search history, browsing history, and activity history. It can also include personally identifying information such as profile information.
\item \textbf{Data Exposure:} This refers to scenarios when a user's personal data is disclosed in a way that is beyond the user's ability to control. This can include sharing personal data with third parties, advertisers, developers, governments, social media, and the public. This includes the notion of selling data to third parties (often for ads) in ways that are opaque to users.
\item \textbf{Data Harms:} Safety concerns arise out of privacy problems when a user's personal data is inaccurate or obsolete. When such data is shared or misused, it can lead to misattribution, which could cause physical or mental harm, such as blackmail or coercion.
\item \textbf{Data Hiding:} In data hiding concerns, users express a desire to explicitly hide their personal data. It can refer to a broad range of data, including calendars, photos, albums, videos, contacts, messages, playlists, notes, etc. They often want to know where the controls are to do so, how they work, and exactly what kind of data hiding is achieved.
\item \textbf{Data Management and Storage:} Data Management and Storage in IoT involves the secure handling, analysis, and transformation of data through various operations, algorithms, and workflows to maintain privacy, integrity, and confidentiality. It also encompasses the reliable retention and protection of data in storage systems, whether on local devices, databases, or cloud platforms, to prevent unauthorized access, data loss, or corruption. Together, these processes ensure that user data is managed and stored with a focus on security, accessibility, and compliance with privacy standards.
\item \textbf{Data Security and Data Theft:} Data security is a privacy problem when accounts or enterprises are breached, and the attacker gathers users' personally identifying information and personal data, which is gathered and/or leaked. The strength of authentication mechanisms has a direct impact on the likelihood of account hacking and, thus, subsequently on the downstream event of private data theft.
\item \textbf{Data Sharing:} This refers to the sharing of personal data that the user can or should be able to control. It includes accidental or unintended sharing when the user inadvertently makes a mistake with the UI or doesn't understand the sharing controls. It also includes forced sharing (when a user is forced to share some data just to use the app or cross-app sharing occurs), and the user does not feel consent was given freely. This can also refer to the types of privacy controls for sharing, such as password protection for photos, files, calendars, etc.
\item \textbf{General Comments Related to Security and Privacy:} Broad observations or reflections on privacy and security practices, policies, or challenges. This theme includes general sentiments, critiques, or concerns about the handling of security and privacy issues, such as overall trust in data protection practices, perceptions of safety, the adequacy of security measures, or the importance of privacy controls. These comments are not tied to specific incidents but reflect overarching views on the effectiveness, transparency, and ethical considerations of security and privacy practices.
\item \textbf{Location Tracking:} The collection of location data that enables location tracking is so widespread that this is its own category. A user's location data can be collected at varying levels of granularity. Privacy controls to limit location tracking are often hard to discover and use in a consistent fashion. Multiple location controls can cause user confusion.
\item \textbf{Personalized Advertising:} When sharing or selling a user's data for advertising purposes is a form of data exposure, this taxonomy item is called out separately because it is known to be very pervasive. Personalized advertising is based on users' data; users sometimes find this unwanted and/or creepy. Sometimes, paid services can be a way to reduce or eliminate ads.
\item \textbf{Policies and Law:} Privacy policies are how apps, IoT services or web services declare the privacy practices they follow to their users. Different countries and jurisdictions around the world have various privacy laws that developers who operate in those countries are liable to adhere to.
\item \textbf{Privacy Controls:} This refers to the privacy controls users employ to hide their personal data to explicitly control data collection or sharing. Privacy controls are sometimes hard to find within a user interface or not sufficiently explained to the user, and the user is not sure exactly what these controls do. Privacy controls or settings are a way to express privacy preferences. This can also include parental controls or refer to controls to download one's personal data.
\item \textbf{Privacy Ethics:} This refers to ethical concerns that arise when privacy data is leaked and personal information is used to offer unequal or biased services to specific groups of people. It also encompasses the moral implications of individuals exhibiting self-righteous attitudes toward privacy, using humor or sarcasm to express privacy concerns, and expressing personal skepticism and opinions about privacy practices. Furthermore, it addresses the ethical dilemma of recognizing privacy concerns while remaining indifferent to their implications and the trade-off between privacy and utility, where individuals may sacrifice their privacy for perceived benefits or conveniences.
\item \textbf{Secure Communication:} Secure communication in IoT refers to the protection of data and services exchanged between devices, which are transferred through various communication patterns, including telemetry, inquiries, notifications, and commands. These communication channels must be secured to ensure the privacy and confidentiality of the information being shared.
\item \textbf{Security Vulnerabilities:} Security Vulnerabilities are weaknesses or points of exposure in IoT devices and systems that can be exploited by attackers to perform malicious actions. In the context of IoT, these vulnerabilities contribute to a broad attack surface, which includes various risks, such as communication attacks, device exploitation, and dynamic attacks. Attackers can leverage these vulnerabilities using a range of tools and malicious code, potentially compromising device integrity, data privacy, and system functionality.
\item \textbf{Software and Firmware Updates:} Software and firmware updates refer to the processes of regularly updating and configuring security features in IoT devices to address emerging threats and vulnerabilities. While many mobile and desktop operating systems automatically perform these updates, IoT devices often receive infrequent updates due to their limited numbers and heterogeneous nature.
\item \textbf{Surveillance:} Surveillance is a privacy concern related to feeling one is being spied on or monitored without awareness or consent. Spying can happen via sensors (such as cameras, microphones, activity sensors, and location trackers) on users' devices. It can also occur from devices users do not control, such as satellites, drones, neighbors' cameras, enterprise audio, and video capture devices, and so on.
\item \textbf{Trust and Transparency:} Trust entails establishing confidence, and assurance in the integrity of systems, services, or interactions, fostering positive relationships and user satisfaction. Transparency refers to how well apps, devices, and services communicate to users what private data they collect, the purpose of the data collection, and how users can control that process.
\item \textbf{Usability:} Ensuring that privacy controls, settings, and interfaces are intuitive, effective, and user-friendly, enhancing user experience and promoting privacy awareness.

\end{enumerate}

==> Section/apdx_themes_src.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\subsection{High-level themes with source information} \label{themesrc}
\begin{table*}[]
\caption{The 85 high-level themes with their sources from prior work, the OSF repository, or empirical observation.}
\centering
\resizebox{0.65\textwidth}{!}{\begin{tabularx}{\textwidth}{@{} XXX @{}}
\toprule
\multicolumn{3}{c}{High-level Themes}                                                                                                                           \\ \midrule
1. access / participation \cite{wang2009privacy}                            & 30. device hacking \cite{akbar2021multicriteria}                           & 59. privacy invasion \cite{akgul2024decade}                                      \\
2. access control \cite{williams2019security,alsamani2018taxonomy,das2018taxonomy}                                    & 31. ease of adoption \cite{wang2009privacy}                         & 60. privacy policies and laws \cite{akgul2024decade}                             \\
3. advertising \cite{akgul2024decade}                                      & 32. eavesdropping \cite{chen2018internet}                            & 61. privacy preservation \cite{das2018taxonomy}                                 \\
4. affiliation with a country or a geographic region \cite{osf} & 33. encryption and confidentiality \cite{williams2019security}          & 62. purpose specification \cite{wang2009privacy}                                \\
5. appropriation \cite{solove2005taxonomy}                                     & 34. fairness (empirical)                                & 63. recognizing privacy concerns but showing indifference (empirical) \\
6. authentication \cite{williams2019security,gulzar2019internet,das2018taxonomy,ogonji2020survey}                                   & 35. fraud (empirical)                                   & 64. remove personally identifiable information \cite{akgul2024decade}           \\
7. authorization \cite{gulzar2019internet,das2018taxonomy}                                    & 36. generic privacy issues \cite{harkous2022hark}                  & 65. responsiveness \cite{wang2009privacy}                                        \\
8. being self-righteous about privacy (empirical)                & 37. generic security issues (empirical)                 & 66. safety \cite{akgul2024decade}                                               \\
9. blackmail \cite{solove2005taxonomy}                                        & 38. government oversight \cite{rizvi2018securing}                    & 67. seclusion \cite{wang2009privacy}                                            \\
10. breach of confidentiality \cite{solove2005taxonomy}                        & 39. humor or sarcasm to express concerns \cite{bhagavatula2022adulthood}     & 68. secure communication \cite{williams2019security}                                 \\
11. business practice transparency (empirical)                  & 40. identification \cite{solove2005taxonomy,ogonji2020survey}                          & 69. selling data \cite{akgul2024decade}                                         \\
12. choice / consent \cite{wang2009privacy}                                & 41. information dissemination \cite{alsamani2018taxonomy}               & 70. software and firmware updates \cite{akbar2021multicriteria}                        \\
13. company's affiliation \cite{osf}                           & 42. information processing \cite{alsamani2018taxonomy}                   & 71. software/hardware bugs \cite{alsubaei2017security}                                \\
14. concerns or vignettes about hackers \cite{osf}              & 43. insecurity \cite{solove2005taxonomy}                               & 72. storage \cite{alsamani2018taxonomy}                                               \\
15. consent \cite{akgul2024decade}                                          & 44. intrusion \cite{solove2005taxonomy}                               & 73. surveillance  \cite{akgul2024decade,solove2005taxonomy}                                        \\
16. data availability \cite{ogonji2020survey}                                & 45. intrusion detection \cite{alqassem2014taxonomy,akbar2021multicriteria}                     & 74. surveillance by a government or a regime \cite{osf}             \\
17. data collection \cite{akgul2024decade}                                  & 46. invasive customer support \cite{osf}               & 75. system/application \cite{alsubaei2017security}                                   \\
18. data confidentiality \cite{ogonji2020survey}                            & 47. issues with apps \cite{osf}                        & 76. technical and technological issues \cite{osf}                    \\
19. data deletion \cite{akgul2024decade}                                   & 48. lack of authentication and authorization \cite{akbar2021multicriteria} & 77. tracking \cite{osf}                                             \\
20. data disclosure \cite{alsubaei2017security}                                 & 49. lack of trust in the device \cite{osf}              & 78. trading privacy for utility (empirical)                           \\
21. data exposure \cite{akgul2024decade}                                    & 50. location and tracking \cite{osf}                   & 79. transparency \cite{ogonji2020survey}                                          \\
22. data integrity \cite{alqassem2014taxonomy,ogonji2020survey}                                   & 51. malware \cite{alsubaei2017security}                                 & 80. trust \cite{rizvi2018securing,ogonji2020survey}                                                \\
23. data minimization \cite{ogonji2020survey}                                & 52. notice / awareness \cite{wang2009privacy}                      & 81. unlinkability \cite{wang2009privacy}                                        \\
24. data misuse (empirical)                                      & 53. onward transfer \cite{wang2009privacy}                          & 82. usability \cite{wang2009privacy}                                            \\
25. data modification \cite{akbar2021multicriteria}                                & 54. password issues \cite{akgul2024decade}                          & 83. use limitation \cite{wang2009privacy}                                        \\
26. data privacy \cite{ogonji2020survey}                                     & 55. payment security \cite{osf}                        & 84. user preference \cite{wang2009privacy}                                      \\
27. data security \cite{osf,akgul2024decade}                                    & 56. personal skepticism and opinions \cite{osf}         & 85. wi-fi security \cite{osf}                                       \\
28. data sharing \cite{akgul2024decade}                                     & 57. physical security \cite{he2023free}                       &                                                           \\
29. decisional interference \cite{solove2005taxonomy}                          & 58. privacy controls \cite{akgul2024decade}                         &                                                           \\ \bottomrule
\end{tabularx}}
\end{table*}

==> Section/apdx_wcountries.tex <==
%\newpage
% \section{Countries from which the reviews were posted in Dataset $\mathcal{W}$} \label{countryw}
% \subsection{Choropleth map}
% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.45\textwidth]{Figure/reviewed_in.pdf}
% \caption{Each color in the choropleth map represents reviews of what product categories are posted from a country. For resolution purposes, Singapore cannot be seen.}
% \label{reviewedin}
% \end{figure}
%\newpage


% \subsection{Number of Reviews by Country}
% \input{Table/countries}

% %\vspace{8pt}
% \section{Choice of GPT-3.5-Turbo}
% \label{sec:gpt35choice}
% We choose GPT-3.5-Turbo to fine-tune our models for several reasons. Firstly, it has the highest token and batch queue limits among all models on OpenAI platform, allowing up to 1 million tokens per minute and 100 million tokens per day for Tier 4 users (as of June 1, 2024)~\cite{openai-ratelimit}, providing flexibility for fast training with large prompts. This information finds support from Ye et al. \cite{ye2023comprehensive}, who argue that it is the most capable among the GPT-3.5-series models (code-davinci-002, text-davinci-002, text-davinci-003, and GPT-3.5-turbo) and is optimized for chat at one-tenth of the cost of text-davinci. Secondly, we see the recent use of GPT-3.5-Turbo in several domains related to information retrieval such as understanding of ultrasound medical reports \cite{wang2024investigation}, combinatorial problem solving \cite{masoud2024exploring}, and extracting information from scientific articles on diabetic retinopathy \cite{gue2024evaluating}. Finally, its performance compared to other models finds support in the work of Addlesee et al. \cite{addlesee2023multi}. The study finds that while multi-party conversations remain challenging for state-of-the-art LLMs, GPT-3.5-Turbo significantly outperformed T5 in few-shot settings, achieving higher accuracy in goal tracking and intent-slot recognition tasks with limited data.

% For obtaining deterministic outputs, we set the \texttt{temperature} parameter to 0 (though we tried other values). To overcome hallucination-induced deviations in the LLM response, we set both \texttt{frequency\_penalty} and \texttt{presence\_penalty} values to 2.

==> Section/apdx_wproducts.tex <==
\section{List of Products from The Wild Dataset $\mathcal{W}$}\label{products}
\subsection{Fitness Tracker: 23 ASINS, 24046 reviews}
\input{Table/p_ft}
\subsection{Smart Speaker: 24 ASINS, 32179 reviews}
\input{Table/p_shs}
%\newpage
\subsection{Security Camera: 28 ASINS, 35524 reviews}
\input{Table/p_sscs}

==> Section/shortsummaryft.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{ltablex}[]
\begin{tabularx}{1.0\textwidth}{@{} p{2cm} X 
@{}}
\toprule
\textbf{Bucket}                                  & \textbf{Fitness Trackers}                                                                                                                                                                                                                                                                                                                                                                                                  e                                                                                                                                        \\ \midrule
Access Control                                   & A significant concern in access control is the app's excessive permission requests, requiring access to extensive personal information like photos, contacts, location, and call history. This lack of granular control over which data is accessed heightens fears of potential data misuse, unauthorized access, and violations of privacy.                                                                                                                                                                                                                      \\
Anonymity                                        & -                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\
Authentication                                   & Users are concerned that the requirement to keep the Zepp app open at all times for Alexa functionality poses authentication-related privacy risks, as it may lead to constant data collection. Additionally, customers are experiencing authentication issues, such as being locked out of the app for 24 hours after two failed login attempts and having to deal with password reset links that expire within two hours.                                                                                                                                        \\
Authorization                                    & The app presents significant authorization concerns by modifying user phone settings without their knowledge or consent—for instance, adding new websites to the "approved" list without permission. Furthermore, purchasing fitness trackers from unauthorized dealers may result in warranty issues, as manufacturers might not honor claims from unapproved sources.                                                                                                                                                                                            \\
Availability                                     & Users are experiencing significant availability issues due to data loss from syncing problems and app malfunctions. Specific reports mention unexplained disappearance of data, loss of two days' worth of data after resolving sync issues by draining the battery, and the app failing to open—leading to a reinstallation that results in account loss and renders the device unusable.                                                                                                                                                                         \\
Confidentiality                                  & There are significant confidentiality concerns that personal data from the fitness tracker may be accessed by unauthorized parties due to vague privacy policies and the app's connections to China. This lack of transparency in data sharing practices raises fears that sensitive information, like sleep data, could be compromised.                                                                                                                                                                                                                           \\
Consent                                          & Users are concerned that their consent is being coerced when they're pressured to grant excessive app permissions or provide sensitive personal information just to access basic device functionality. This raises questions about the validity of their consent, as they feel compelled to agree to intrusive data collection practices simply to use the devices they have purchased.                                                                                                                                                                            \\
Data Accuracy                                    & Many reviewers report significant inaccuracies in fitness trackers' data, including step counts, calorie burn estimations, heart rate readings, and sleep tracking, with instances like blood pressure readings being markedly lower than calibrated measurements. This lack of data accuracy raises serious safety concerns, as users might unknowingly rely on faulty health metrics for important decisions, and coupled with invasive data collection practices, there's a risk that inaccurate health information could be collected and potentially misused. \\
Data Collection                                  & Users are concerned that the fitness tracker and its app collect excessive personal information—such as location, contacts, call logs, and credit card details—which may be exploited for profit or surveillance. The lack of transparency about how this data is used and shared, particularly due to the app's connections with Chinese companies, heightens distrust and anxiety over potential misuse of sensitive personal information.                                                                                                                       \\
Data Deletion                                    & Users are concerned that their data may not be fully deleted even after requesting account deletion or uninstalling apps, leaving sensitive information vulnerable to misuse. Additionally, accidental data loss due to software glitches or user errors, such as disappearing data or syncing issues, is a significant concern.                                                                                                                                                                                                                                   \\
Data Exposure                                    & Users have expressed concerns about data exposure when purchasing Fitbit devices from unauthorized third-party resellers, fearing that these sellers might access their data or provide counterfeit devices with compromised security features. Additionally, there are worries about the app's invasive data collection practices and the company's potential sharing of user information with third parties, including data brokers.                                                                                                                             \\
Data Harms                                       & Users are reporting psychological harm due to inaccurate or potentially manipulated data from fitness trackers, such as concerns that health metrics are being inflated after a subscription lapse to encourage renewals. Additionally, reports of physical discomfort, including skin irritation and speculation about radiation exposure from the devices, highlight the need for greater transparency and safety in data handling and device usage.                                                                                                             \\
Data Hiding                                      & -                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\
Data Management and Storage                      & Users are concerned about the security of personal data collected by fitness trackers, citing fears of unauthorized access or data breaches due to a lack of transparency in how the data is stored and managed. Additionally, issues like syncing problems, app malfunctions, and difficulties transferring data between devices raise concerns about the reliability of data storage and the potential for permanent data loss.                                                                                                                                  \\
Data Security and Data Theft                     & Users are highly concerned about data security due to the app requiring storage of credit card information for "free" trials and subscriptions, leading to reports of unauthorized charges and account compromises. The absence of clear security measures and the app's connections to Chinese companies further amplify fears of large-scale data breaches and the potential misuse of sensitive personal and health data.                                                                                                                                       \\
Data Sharing                                     & Users are concerned about the app's lack of transparency and control over their personal data, fearing it may be shared with third parties, sold to data brokers, or used for purposes beyond fitness tracking like targeted advertising or research. These worries are amplified by the app's connection to Chinese companies, leading to unease about the potential sharing of their data with the Chinese government or other entities.                                                                                                                         \\
General Comments Related to Security and Privacy & Users express widespread concerns about the security and privacy of fitness tracker apps, highlighting issues such as excessive personal data collection, lack of transparency in data usage, and the potential for data breaches or misuse of information. These fears are intensified by the apps' connections to companies in certain countries, leading to apprehension about data sharing with foreign governments, and are compounded by reports of phishing scams, unauthorized charges, and other malicious activities experienced after using the apps.   \\
Location Tracking                                & Users are concerned that fitness tracker apps demand constant access to their location data, even when GPS features are not being used, fearing that their movements are being tracked and sensitive location information is being collected. This continuous location tracking, combined with vague privacy policies and connections to Chinese companies, heightens anxieties about potential data misuse, surveillance, and the unauthorized sharing of location data with third parties.                                                                       \\
Personalized Advertising                         & Users are frustrated with the fitness tracker app's aggressive personalized advertising, including frequent pop-up ads promoting additional products and services—even for those who have already purchased the device. This intrusive approach not only disrupts the user experience but also raises privacy concerns due to the potential reliance on extensive data collection and analysis for ad personalization.                                                                                                                                             \\
Policies and Law                                 & Users are concerned that Fitbit's data collection practices and lack of transparency in its privacy policies may violate consumer protection laws by not providing adequate control over personal information. Additionally, the requirement to use proprietary charging cables and potential warranty issues could infringe upon consumer rights under applicable laws.                                                                                                                                                                                           \\
Privacy Controls                                 & Users are frustrated by the lack of control over privacy settings, particularly the inability to customize notifications and limit data sharing with third parties. They express concerns about sensitive personal information being displayed without consent and the absence of parental controls to prevent children from receiving unwanted notifications.                                                                                                                                                                                                     \\
Privacy Ethics                                   & Users express privacy ethics concerns regarding Fitbit's use of manipulative design tactics, such as requiring excessive permissions and persistently pressuring them to provide credit card information despite prior refusals. Additionally, there is unease about the potential misuse of sensitive health data for marketing or profit-driven purposes, which may compromise user privacy.                                                                                                                                                                     \\
Secure Communication                             & Users are concerned that the device's always-on Bluetooth requirement for syncing and accessing features could pose security risks in terms of secure communication. They fear that this continuous connection may expose their personal data to unauthorized access or interception, especially given anxieties about the app's data collection practices and its connections to Chinese companies.                                                                                                                                                               \\
Security Vulnerabilities                         & Users are concerned that fitness trackers and their associated apps may have security vulnerabilities that could be exploited by hackers and malware, potentially leading to data theft, financial fraud, and device malfunctions. Reports of suspicious activities such as browser lag, app freezing, unauthorized access to connected devices like Alexa, and fraudulent transactions have heightened anxieties about the security of these devices and the potential for exploitation by malicious actors.                                                      \\
Software and Firmware Updates                    & Users are concerned that software and firmware updates may introduce new security vulnerabilities or worsen existing ones, with incidents like devices becoming "bricked" during updates highlighting these risks. Additionally, frequent and intrusive update requests without clear information about their purpose and content have led to user frustration.                                                                                                                                                                                                    \\
Surveillance                                     & Users are concerned that the app's extensive collection of personal data—such as sleep patterns, location, and heart rate—could lead to surveillance or misuse by third parties without their consent. Specifically, worries about the app's connections to Chinese companies raise fears that data might be shared with the Chinese government or other entities for surveillance or malicious purposes.                                                                                                                                                          \\
Trust and Transparency                           & Many users feel misled by Fitbit because of ambiguous marketing around subscription requirements and the true costs of accessing the device's full functionality. This lack of transparency, combined with frequent updates that change app features, has eroded trust and made it challenging for users to assess the security and privacy implications of using the device.                                                                                                                                                                                      \\
Usability                                        & Constant requests for sensitive information like credit card details and location access, combined with unclear instructions and complex navigation, lead users to view these usability issues as intrusive attempts to access their data. This poor usability undermines trust, making it difficult for users to understand and manage privacy settings and data sharing options.                                                                                                                                                                                 \\ \bottomrule
\end{tabularx}
\end{ltablex}

==> Table/SummaryWithReviews.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{comment}
\begin{table*}[]
\caption{Summary of the top five high level themes per device category with example reviews}
\begin{tabularx}{\textwidth}{@{} p{1cm}  p{3cm} X X  @{}}
\toprule
\textbf{Device type}  & \textbf{High-level Theme}               & \textbf{Summary of the Theme} & \textbf{Example Review(s)} \\ \midrule
\multirow{5}{*}{Trackers} & Data Security and Data Theft & Users express significant worry about data security due to the app's requirement to store credit card information for `free' trials, leading to reports of unauthorized charges and account breaches. Fears are heightened by unclear security measures and when app's are tied to Chinese companies, raising worries about large-scale breaches and misuse of sensitive data.           & "Shortly after using this and giving it all the permissions and ask for there were mysterious charges on my debit card", "About 5 minutes after downloading the app for this watch, my phone was blowing up with scam texts."                 \\ \hline
                          & Privacy Controls             & Summary          & Review                  \\ \hline 
                          & Data Collection              & Summary          & Review                  \\
                          & Usability                    & Summary          & Review                  \\
                          & Authentication               & Summary          & Review                  \\ \midrule
\multirow{5}{*}{Speakers} & Surveillance                 & Summary          & Review                  \\
                          & Authentication               & Summary          & Review                  \\
                          & Authorization                & Summary          & Review                  \\
                          & Access Control               & Summary          & Review                  \\
                          & Privacy Controls             & Summary          & Review                  \\ \midrule
\multirow{5}{*}{Cameras}  & Surveillance                 & Summary          & Review                  \\
                          & Privacy Controls             & Summary          & Review                  \\
                          & Usability                    & Summary          & Review                  \\
                          & Data Security and Data Theft & Summary          & Review                  \\
                          & Access Control               & Summary          & Review                  \\ \bottomrule
\end{tabularx}
\end{table*}
\end{comment}

\begin{table*}[!h]
\small
\caption{Summary of the top five high level themes, with sample quotes, for fitness trackers.}
\vspace{-4pt}
\begin{tabularx}{\textwidth}{p{2cm}  p{7cm} X @{}}
\toprule
 \textbf{High-level Theme}               & \textbf{Compact Theme Summary} & \textbf{Example Review(s)} \\ \midrule
Data Security and Data Theft (12.5\%) & Users express significant worry about apps that requirement credit card information for `free' trials, as they fear it can lead to reports of unauthorized charges and account breaches.          & "\textit{Shortly after using this and giving it all the permissions and ask for there were mysterious charges on my debit card}..." \newline \textit{"About 5 minutes after downloading the app for this watch, my phone was blowing up with scam texts"}.                 \\ \hline
Privacy Controls (10\%)             & Users are frustrated by limited privacy
controls, to customize notifications (especially when they display sensitive data), and to restrict
third-party data sharing.          & \textit{"I hate that it shows what day of my menstrual cycle I’m on. How
embarrassing. . . no way to remove that"}.                   \\ \hline 
Data Collection (9\%)              & Users worry that fitness trackers and
their apps collect excessive personal data—like location, contacts,
call logs, and credit card details—raising fears of exploitation for
profit or surveillance. Concerns are amplified by lack of transparency for some apps.         & \textit{"The thing would not even tell time, unless you register an account
and provided personal information to a company in [COUNTRY-NAME]. If I
buy something like a watch, I expect it to work without me having
to give out any personal information"}                 \\ \hline
Usability (7\%)                    & Users find frequent requests for sensitive data,
like credit card details and location, paired with unclear instructions
and complex navigation. This complicates
managing privacy settings and data sharing.          & \textit{"The [PRODUCT NAME] has two flaws that are deal breakers for me. 1: you cannot change the apps that display on the face -
so if someone was looking at my watch they could see my weight.
I am a teacher, my students play with my watch at times and I
don’t need them to know that personal information".}                  \\ \hline
Authentication (6\%)               &   Customers talk about authentication
issues, including 24-hour lockouts after two failed logins and password reset links expiring within two hours. Users are also concerned that keeping an app constantly active to enable voice assistant functionality may pose privacy risks, including potential continuous data collection        &  \textit{"I forgot which password I was using with the app and logged in with the wrong one 2x. I reset the password and then received a
message at my next login attempt that I wouldn’t be able to login
for 24 hours because of too many attempts - WHAT??? That is
crazy! I understand the need for security, but that is an excessive
amount of time to be locked out of an account."}                   \\ 
\bottomrule
\end{tabularx}
\label{tab:top-themes-trackers}
\vspace{-16pt}
\end{table*}


\begin{table*}[!h]
\small
\caption{Summary of the top five high level themes, with sample quotes, for smart speakers.}
\vspace{-4pt}
\begin{tabularx}{\textwidth}{p{2cm}  p{7cm} X @{}}
\toprule
 \textbf{High-level Theme}               & \textbf{Compact Theme Summary} & \textbf{Example Review(s)} \\ \midrule
Surveillance (17\%) &    Users are deeply anxious about the ‘always-
on’ nature of smart speakers, fearing constant surveillance through
continuous conversation recording and data sharing with manufacturers, the government, or third parties. Concerns are heightened by
unexpected activations without a clear wake word.    & \textit{"You can believe the stories you hear about [PRODUCT-NAME] listening, We would talk about something and it would appear in
your news feed advertisements. Scary. Unplugged it.}." \newline \textit{"...there is a HUGH security question looming with the IoT hacking by our government, political parties, other nations and bad actors looking to make a quick buck. This is an ongoing threat."}                 \\ \hline

Authentication (10.5\%)             &  Users voice that unauthorized access to user accounts and devices presents a major authentication risk, as seen in cases where scammers impersonate as vendor technicians to steal personal information through remote access. Furthermore, instances of devices being linked to incorrect or outdated accounts reveal weaknesses in account linking and authentication processes.    &  "\textit{I used the pop up virtual assistant during setup who remoted into my computer, and installed a network security program. Two days later I got 8 calls about fraudulent charges on my account."} \newline "\textit{I was eager to set it up. Process started fine but went oddly haywire right away. [PRODUCT] opened with my daughter’s name and email pre-entered in the owner ID. That’s weird, since our daughter has not lived here for decades. }" \               \\ \hline 
Authorization (10\%)              &  Users face authorization concerns with
smart speakers due to unintended activations from TV commercials,
background noise, or other voices, risking unauthorized actions
and data access. Shared accounts further exacerbate risks, allowing
others to view personal data, make purchases, or control devices,
underscoring the need for stronger authorization mechanisms.   & \textit{"apparently while I was asleep I woke up for a few
minutes but wasn’t really coherent, idk what I said if anything to
activate the controller device however, it recorded several
minutes of me babbling on about dropping my medication box
all over the floor. It used my contacts to send that voice message to everyone in my contacts. My friends called to ask what was going on. Be careful ppl. I deregistered several devices."}                 \\ \hline
Access Control (8\%)                    &     Users find managing shared or multiple accounts challenging, and find these situations risk unauthorized access    & \textit{"Beware! if you gift this item to someone and don’t select "gift" when purchasing, the device will be linked to your account automatically. UNLESS the recipient "deregisters" it. Our daughter tried to create her own account but I was charged ... even though I never approved it".}                  \\ \hline
Privacy Controls (7.5\%)               &   Users raised concerns about available
privacy controls on smart speaker devices stating, that they tried privacy controls like unplugging the device, disabling features, and deleting recordings. However,many found these measures difficult to use or inadequate.     &  \textit{"I feel its a bit intrusive with recording what i say and storing it. i absolutely hate that so i unplug mine when I'm not around which defeats the entire purpose. I also wish privacy and security options allowed further control. Like, I want to say a family member can access on this information at said time on said network."}                   \\ 
\bottomrule
\end{tabularx}

\label{tab:top-themes-speakers}
\vspace{-16pt}
\end{table*}


\begin{table*}[!h]
\small
\caption{Summary of the top five high level themes, with sample quotes, for security cameras.}
\vspace{-4pt}
\begin{tabularx}{\textwidth}{p{2cm}  p{7cm} X @{}}
\toprule  \textbf{High-level Theme}   & \textbf{Compact Theme Summary} & \textbf{Example Review(s)} \\ \midrule
Surveillance (17\%) &    Users worry that security cameras may
enable unauthorized surveillance by strangers, landlords, or even
family members without their knowledge or consent. They also
feel uneasy about the lack of control motion
detection or recording, leading to a sense of constant monitoring
and diminished privacy at home.   & \textit{"I purchased these so that I could spy on my stepson and his lazy girlfriend, they gonna calm down and stop getting into my stuff I promise because now I can see everything y’all
do even when we’re gone"}. \newline \textit{"I surely hope to never find
our landlord sneaking in when we are not home as we heard he is
nosy and goes in tenants apartments."}                 \\ \hline

Privacy Controls (12\%)             &  Users feels they cannot manage the sense of constant surveillance due to the lack of
detailed privacy controls. They also worry about limited
control over data sharing, fearing that vendors may share personal
information with third parties or authorities without consent.    & \textit{"I purchased 4 minicams but I'm not happy. The cameras lack basic features like not being able to share access to the cameras with others without supplying them your user credentials."}                  \\ \hline 
Usability (10\%)              &   A major usability issue is the slow and lagging
performance of the apps and cameras, causing missed events, delayed notifications, and difficulty accessing live feeds. The user experience is complicated by non user-friendly interfaces, poor documentation, confusing setup processes and limited control over camera settings.   & \textit{"When you get alerts on your phone about motion detection, there’s
no way to disable individual cameras - you can disable all or
enable all. You can’t opt out for just individuals. So if one shows
the passing cars and people, you can't disable notifications just for the cars, while getting them for the people."}                 \\ \hline
Data Security and Data Theft (8\%)     &   Users are concerned about
encryption issues with local SD card storage, which is vulnerable to
theft and lacks automatic backups. They also worry about potential
hacking and unauthorized account access, underscoring the need
for stronger security measures.     & \textit{"I have no intention of subscribing to the cloud. On forums they say that even with just local usb storage, people can still view clips with the app."} \newline \textit{"I placed this to keep tabs on my landlord entering my room when I’m not home. Not a week had passed by when
I received an email from hacker saying they have private
recordings of me and that I need to pay they’ll send them to my contacts."}                  \\ \hline
Access Control (7\%)    &    Many home security camera systems lack
granular access control, preventing users from assigning different
permission levels to multiple users. Forcing them to share full
administrative credentials with individuals who only need limited
viewing, poses risks due to potential
unauthorized changes and deletions.  &  \textit{"The only way to share access to your live videos is by giving
your username and password to a person. The individual then has
access to change your email address, password, and delete videos.
Technically, they can lock you out of your own security system.
Good luck with that if you have teenagers."} \\ \bottomrule
\end{tabularx}
\label{tab:top-themes-cameras}
\vspace{-16pt}
\end{table*}


==> Table/chisq.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]

\centering
\caption{At the top: Calculation of the concern ratio. In the middle: test for equality of proportions. $H_{0}:$ $|C_{c}|/|R_{c}|$ is the same in each $c$. $H_{A}:$ At least one $|C_{c}|/|R_{c}|$ for a $c$ is different from the others. At the bottom: Posthoc pairwise comparison of the proportions of all pairs of $|C_{c}|/|R_{c}|$-s. The significance code *** means $p < .001$.}
\resizebox{0.65\textwidth}{!}{\begin{tabular}{|lllll|}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Category}}} & \multicolumn{4}{c|}{\textbf{Concern ratio calculation}}                                                                                                       \\ \cline{2-5} 
\multicolumn{1}{|l|}{}                                   & \multicolumn{1}{l|}{\textbf{No. of reviews with concerns}} & \multicolumn{1}{l|}{\textbf{Total no. of reviews}} & \multicolumn{2}{l|}{\textbf{Concern ratio}} \\ \hline
\multicolumn{1}{|l|}{FT}                                 & \multicolumn{1}{l|}{505}                                   & \multicolumn{1}{l|}{23894}                         & \multicolumn{2}{l|}{0.0211}                 \\
\multicolumn{1}{|l|}{SHS}                                & \multicolumn{1}{l|}{847}                                   & \multicolumn{1}{l|}{32069}                         & \multicolumn{2}{l|}{0.0264}                 \\
\multicolumn{1}{|l|}{SSCS}                               & \multicolumn{1}{l|}{3544}                                  & \multicolumn{1}{l|}{35186}                         & \multicolumn{2}{l|}{0.1007}                 \\ \hline
\multicolumn{5}{|c|}{\textbf{Test for equality of proportion}}                                                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{\textbf{Type of test}}              & \multicolumn{1}{l|}{\textbf{Test statistic}}               & \multicolumn{1}{l|}{\textbf{$df$}}                   & \multicolumn{2}{l|}{\textbf{$p$-value}}       \\ \hline
\multicolumn{1}{|l|}{Chi-squared}                        & \multicolumn{1}{l|}{$\chi^{2}$ = 2498.9}                    & \multicolumn{1}{l|}{2}                             & \multicolumn{2}{l|}{\textless 2.2e-16***}      \\ \hline
\multicolumn{5}{|c|}{\textbf{Pairwise comparison}}                                                                                                                                                                       \\ \hline
\multicolumn{1}{|l|}{\textbf{$C_{i}$}}                        & \multicolumn{1}{l|}{\textbf{$C_{j}$}}                           & \multicolumn{3}{l|}{\textbf{$p$-value}}                                                            \\ \hline
\multicolumn{1}{|l|}{FT}                                 & \multicolumn{1}{l|}{SHS}                                   & \multicolumn{3}{l|}{2e-04***}                                                                       \\
\multicolumn{1}{|l|}{FT}                                 & \multicolumn{1}{l|}{SSCS}                                  & \multicolumn{3}{l|}{\textless 2e-16***}                                                                    \\
\multicolumn{1}{|l|}{SHS}                                & \multicolumn{1}{l|}{SSCS}                                  & \multicolumn{3}{l|}{\textless 2e-16***}                                                                    \\ \hline
\end{tabular}
\label{chisquaredtable}
}

\end{table*}

==> Table/chisq2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[!h]
\caption{At the top: Calculation of the concern ratio. In the middle: test for equality of proportions. $H_{0}:$ $|C_{c}|/|R_{c}|$ is the same in each $c$. $H_{A}:$ At least one $|C_{c}|/|R_{c}|$ for a $c$ is different from the others. At the bottom: Posthoc pairwise comparison of the proportions of all pairs of $|C_{c}|/|R_{c}|$-s. The significance code *** means $p < .001$.
\das{either make the table take up full page width and add the proportions and chi test in the same same table or do two separate tables. Current vertical one table is hard to parse}}
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Category}}} & \multicolumn{3}{c}{\textbf{Concern Ratio Calculation}}              \\ \cmidrule(l){2-4} 
\multicolumn{1}{l|}{}                                   & \textbf{$|C_{c}|$}               & \textbf{$|R_{c}|$}   & \textbf{$|C_{c}|/|R_{c}|$}          \\ \midrule
\multicolumn{1}{l|}{FT}                                 & 505                       & 23894         & 0.0211                  \\
\multicolumn{1}{l|}{SHS}                                & 847                       & 32069         & 0.0264                  \\
\multicolumn{1}{l|}{SSCS}                               & 3544                      & 35186         & 0.1007                  \\ \midrule
\multicolumn{4}{c}{\textbf{Test for Equality of Proportion}}                                                                  \\ \midrule
\textbf{Test}                                           & \textbf{Test Statistic}   & \textbf{$df$}   & \textbf{p-value}        \\ \midrule
Chi-squared                                             & $\chi^{2} = 2498.9$             & 2             & \textless{}2.2e-16***   \\ \midrule
\multicolumn{4}{c}{\textbf{Pairwise Comparison}}                                                                              \\ \midrule
$c_{i}$                                                      & \multicolumn{1}{l|}{$c_{j}$}   & \multicolumn{2}{r}{$p$-value}             \\ \midrule
FT                                                      & \multicolumn{1}{l|}{SHS}  & \multicolumn{2}{r}{2e-04***}            \\
FT                                                      & \multicolumn{1}{l|}{SSCS} & \multicolumn{2}{r}{\textless{}2e-16***} \\
SHS                                                     & \multicolumn{1}{l|}{SSCS} & \multicolumn{2}{r}{\textless{}2e-16***} \\ \bottomrule
\end{tabular}
\label{chisquaredtable}
\end{table}

==> Table/countries.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\resizebox{0.43\textwidth}{!}{\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{Reviewed in} & \multicolumn{1}{l}{\textbf{FT}} & \multicolumn{1}{l}{\textbf{SHS}} & \multicolumn{1}{l}{\textbf{SSCS}} & \multicolumn{1}{l}{\textbf{Total}} \\ \midrule
United States \worldflag{US}        & 23060                           & 31526                            & 33479                             & 88065                              \\
Canada \worldflag{CA}               & 330                             & 451                              & 696                               & 1477                               \\
United Kingdom \worldflag{GB}      & 421                             & 18                               & 734                               & 1173                               \\
Italy \worldflag{IT}               & 104                             & -                                & 227                               & 331                                \\
Germany \worldflag{DE}              & 86                              & 1                                & 160                               & 247                                \\
Mexico \worldflag{MX}               & 2                               & 163                              & 66                                & 231                                \\
Spain  \worldflag{ES}              & 17                              & 1                                & 124                               & 142                                \\
France \worldflag{FR}               & 12                              & -                                & 29                                & 41                                 \\
India \worldflag{IN}             & -                               & 13                               & -                                 & 13                                 \\
Japan  \worldflag{JP}              & 10                              & -                                & -                                 & 10                                 \\
Australia  \worldflag{AU}          & -                               & 2                                & 8                                 & 10                                 \\
Singapore  \worldflag{SG}          & 2                               & 2                                & 1                                 & 5                                  \\
Brazil  \worldflag{BR}             & 2                               & 2                                & -                                 & 4                                  \\ \bottomrule
\end{tabular}}
\caption{Distribution of reviews across different regions. Region is identified based on the user metadata provided by Amazon.}
\label{tab:country}
\end{table}

==> Table/delta.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!t]
\centering
\caption{Comparison of NLP-based analysis of user comments or reviews in prior works versus our study. \das{use the full horizontal space to reduce the height of the table. Task column can expand side way}}
\resizebox{.8\textwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\toprule
\textbf{Reference} & \textbf{Task}                                                 & \textbf{Text}                                                 & \textbf{Model used}                                                                  & \textbf{\begin{tabular}[c]{@{}l@{}}Use of \\ Taxonomy\end{tabular}}           & \textbf{\begin{tabular}[c]{@{}l@{}}Prompt \\ engineering\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Ratings\\ analysis \end{tabular}} \\ \midrule
Henao et al. \cite{henao2021transfer}     & \begin{tabular}[c]{@{}l@{}}Mining feature \\ requests and \\ bug reports\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}User \\ comments\end{tabular}      & \begin{tabular}[c]{@{}l@{}}BERT\\ (monlingual + \\ multilingual)\end{tabular}        & No                                                                            & No                                                                     & No                                                                                                   \\ \hline
Palomba et al. \cite{palomba2017recommending} & \begin{tabular}[c]{@{}l@{}}Recommending \\ and localizing \\ change requests \end{tabular}                           & \begin{tabular}[c]{@{}l@{}}App \\ reviews\end{tabular}        & \begin{tabular}[c]{@{}l@{}}Classical NLP\\ (Text + \\ Sentiment analysis)\end{tabular}& No                                                                            & No                                                                     & No                                                                                                   \\ \hline
Fu et al. \cite{fu2013people} & \begin{tabular}[c]{@{}l@{}}Users' \\ likes or dislikes \\ toward apps \end{tabular}                           & \begin{tabular}[c]{@{}l@{}}App \\ reviews\end{tabular}        & \begin{tabular}[c]{@{}l@{}}LDA\end{tabular}& No                                                                            & No                                                                     & Yes                                                                                                   \\ \hline
de Ara\'ujo et al. \cite{de2021re} & \begin{tabular}[c]{@{}l@{}}Identification \\ of software \\ requirements\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}App \\ reviews\end{tabular}        & BERT                                                                                 & No                                                                            & No                                                                     & No                                                                                                   \\ \hline
Harkous et al. \cite{harkous2022hark}   & \begin{tabular}[c]{@{}l@{}}Eliciting \\ privacy \\ concerns\end{tabular}                                        & \begin{tabular}[c]{@{}l@{}}App \\ reviews\end{tabular}        & \begin{tabular}[c]{@{}l@{}}T5 with \\ hypothesis based \\ NLI technique\end{tabular} & \begin{tabular}[c]{@{}l@{}}Privacy \\ taxonomies\end{tabular}                 & No                                                                     & No                                                                                                   \\ \hline
Akgul et al. \cite{akgul2024decade}     & \begin{tabular}[c]{@{}l@{}}Analyzing \\ decade-long \\ privacy concerns \\ in app reviews\end{tabular}          & \begin{tabular}[c]{@{}l@{}}App \\ reviews\end{tabular}        & \begin{tabular}[c]{@{}l@{}}T5 \\ architecture \\ with static \\ prompt\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Privacy \\ taxonomies\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}Yes \\ (static)\end{tabular}                & No                                                                                                   \\ \hline
Our work               & \begin{tabular}[c]{@{}l@{}}Mining security \\ and privacy \\ concerns in \\ IoT product \\ reviews\end{tabular} & \begin{tabular}[c]{@{}l@{}}IoT product\\ reviews\end{tabular} & 
gpt-3.5-turbo                                                                        & \begin{tabular}[c]{@{}l@{}}Security \\ and privacy \\ taxonomies\end{tabular} & \begin{tabular}[c]{@{}l@{}}Yes \\ (dynamic)\end{tabular}               & Yes                                                                                                  \\ \bottomrule
\end{tabular}}
\label{tab:comparison-prior-work}

\end{table*}

==> Table/levtest.tex <==
\begin{table}[!t]
\centering
\caption{Levene's test for equality in variances. $H_{0}: \sigma^{2}_{c} = \sigma^{2}_{n}$ vs $H_{A}: \sigma^{2}_{c} \neq \sigma^{2}_{n}$.  $s^{2}_{c}$ and $s^{2}_{n}$ are the sample variances in the ratings of the concern and non-concern reviews, respectively. The significance code ***, and * means $p < .001$ and $p < .05$, respectively.}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{llllllll}
\toprule
\textbf{Device} & \multirow{2}{*}{\textbf{$s^{2}_{c}$}} & \multirow{2}{*}{\textbf{$s^{2}_{n}$}} & \multirow{2}{*}{\textbf{$k$}} & \multirow{2}{*}{\textbf{$n$}} & $F$  & $F-value$ & \textbf{$Pr(\textgreater{}F$)} \\ 
\textbf{type} &  & &  & & distribution &  & \\
\midrule
FT                   & 2.32         & 2.53         & 2          & 23894        & $F_{1, 23892}$                 & 6.2186           & 0.01265*                       \\
SHS                  & 1.77         & 1.25         & 2          & 32069       & $F_{1, 32067}$                & 61.578           & $4.388e-15$***                   \\
SSCS                 & 2.62        & 2.07         & 2          & 35186        & $F_{1, 35184}$                 & 355.77           & $\textless 2.2e-16$***                   \\ 
Overall                 & 2.60         & 1.99         & 2          & 91149        & $F_{1, 91147}$                 & 660.57           & $\textless 2.2e-16$***                   \\ 
\hline
\end{tabular}}
\label{levenetest}

\end{table}

==> Table/longtabletest.tex <==

\begin{xltabular}{\textwidth}{p{1.6cm}XXX}
\caption{Summaries of S\&P concerns found in the reviews of trackers, speakers, and cameras across 28 high-level themes related to security and privacy. The summaries have been generated with NotebookLM. Cells with ``-" imply the TM model did not map any low-level theme in that category with that high-level theme.}
\label{tab:long} 
\hline \multicolumn{1}{c}{\textbf{Theme}} & \multicolumn{1}{c}{\textbf{Trackers}} & \multicolumn{1}{c}{\textbf{Speakers}} &
\multicolumn{1}{c}{\textbf{Cameras}}
\\ \hline 
\endfirsthead

\multicolumn{4}{c}%
{\tablename\ \thetable{} -- continued from previous page} \\
\hline \multicolumn{1}{c}{\textbf{Theme}} & \multicolumn{1}{c}{\textbf{Trackers}} & \multicolumn{1}{c}{\textbf{Speakers}} &
\multicolumn{1}{c}{\textbf{Cameras}}
\\ \hline 
\endhead

\hline \multicolumn{4}{r}{{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot

Access Control                                   & A significant concern in access control is the app's excessive permission requests, requiring access to extensive personal information like photos, contacts, location, and call history. This lack of granular control over which data is accessed heightens fears of potential data misuse, unauthorized access, and violations of privacy.                                                                                                                                                                                                                      & Users have raised concerns about the insufficient granular access control in the [VOICE ASSISTANT] ecosystem, noting that devices can be unintentionally activated by unauthorized users or even voices from TV commercials. Additionally, they face challenges in managing shared accounts to prevent unauthorized access to personal information and device functionalities, especially in households with multiple users.                                                                                                                      & Many home security camera systems lack granular access control, preventing users from assigning different permission levels to multiple users. This forces them to share full administrative login credentials with individuals who only need limited viewing access, raising significant security risks due to potential unauthorized changes and deletions.                                                                                                                                                                                                                                                                                                                                \\ \midrule
Anonymity                                        & -                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & Requiring a cell phone number for [VOICE ASSISTANT] registration compromises user anonymity by fixing the caller ID to that specific number. This linkage associates the user's identity with the device and potentially exposes their phone number to third parties during communications.                                                                                                                                                                                                                                                       & Anonymity is compromised when IP-based location verification inaccurately disables features like facial recognition for users outside restricted areas, inadvertently revealing their location discrepancies. Additionally, audible clicks and visible lights from active cameras alert individuals to surveillance, undermining covert operations and compromising users' desire for anonymous security measures.                                                                                                                                                                                                                                                                           \\ \midrule
Authentication                                   & Users are concerned that the requirement to keep the [APP] open at all times for [VOICE ASSISTANT] functionality poses authentication-related privacy risks, as it may lead to constant data collection. Additionally, customers are experiencing authentication issues, such as being locked out of the app for 24 hours after two failed login attempts and having to deal with password reset links that expire within two hours.                                                                                                                                        & Unauthorized access to user accounts and devices poses a significant authentication risk, exemplified by scammers impersonating [COMPANY] technicians to gain remote access and steal personal information. Additionally, incidents of [DEVICE] being linked to incorrect or outdated accounts highlight vulnerabilities in account linking and authentication processes.                                                                                                                                                            & Users are concerned about the absence of two-factor authentication, which leaves their accounts vulnerable to unauthorized access. Additionally, they experience difficulties with authentication methods—for example, verification codes are sent to outdated phone numbers or require access to devices located elsewhere—hindering their ability to log in and use their camera systems.                                                                                                                                                                                                                                                                                                  \\ \midrule
Authorization                                    & The app presents significant authorization concerns by modifying user phone settings without their knowledge or consent—for instance, adding new websites to the "approved" list without permission. Furthermore, purchasing fitness trackers from unauthorized dealers may result in warranty issues, as manufacturers might not honor claims from unapproved sources.                                                                                                                                                                                            & Users have significant authorization concerns with [VOICE ASSISTANT] devices due to unintended activations caused by commercials, background noise, or other people's voices, leading to actions without explicit user commands and raising risks of unintended data access and privacy violations. Additionally, the broad access granted to shared accounts allows others to potentially view personal information, make unauthorized purchases, or control smart home devices, highlighting the need for more robust authorization mechanisms. & The inability to grant differentiated access forces account owners to share full administrative control with all users, including the ability to view all cameras and modify system settings. This lack of granular authorization poses significant security risks, as anyone with the login credentials can access sensitive features and potentially delete important footage, especially when temporary access is given to individuals like pet sitters or house cleaners.                                                                                                                                                                                                                \\ \midrule
Availability                                     & Users are experiencing significant availability issues due to data loss from syncing problems and app malfunctions. Specific reports mention unexplained disappearance of data, loss of two days' worth of data after resolving sync issues by draining the battery, and the app failing to open—leading to a reinstallation that results in account loss and renders the device unusable.                                                                                                                                                                         & Users are concerned about availability issues stemming from technical glitches and device malfunctions that lead to data loss, such as losing all saved reminders after an Echo device unintentionally resets to factory settings. Additionally, the lack of offline functionality affects availability, with users needing to reprogram devices like smart plugs after unplugging and replugging them.                                                                                                                               & Many home security camera systems face significant availability issues, with users reporting cameras going offline, failing to record events, and experiencing delays in live feeds, which compromises their effectiveness for security purposes. Additionally, the requirement of paid subscriptions to access recorded footage further limits the availability of crucial evidence for users who choose not to pay recurring fees.                                                                                                                                                                                                                                                         \\ \midrule
Confidentiality                                  & There are significant confidentiality concerns that personal data from the fitness tracker may be accessed by unauthorized parties due to vague privacy policies and the app's connections to [GEOGRAPHIC LOCATION]. This lack of transparency in data sharing practices raises fears that sensitive information, like sleep data, could be compromised.                                                                                                                                                                                                                           & Users have significant confidentiality concerns about devices like [VOICE ASSISTANT] unintentionally disclosing personal information, such as misinterpreting conversations and initiating unintended actions like calling emergency services. There is also apprehension that conversations recorded by the device could be accessed by unauthorized parties, raising serious privacy and data security issues regarding personal interactions and stored data.                                                                                  & The main confidentiality concern is the potential for unauthorized third parties to access user data, including sensitive personal information and camera recordings. This risk is heightened by vendors' lack of transparency about their data security practices and the absence of protections like end-to-end encryption.                                                                                                                                                                                                                                                                                                                                                                \\ \midrule
Consent                                          & Users are concerned that their consent is being coerced when they're pressured to grant excessive app permissions or provide sensitive personal information just to access basic device functionality. This raises questions about the validity of their consent, as they feel compelled to agree to intrusive data collection practices simply to use the devices they have purchased.                                                                                                                                                                            & Users, particularly children, may unknowingly consent to subscriptions or purchases through voice interactions with [VOICE ASSISTANT], leading to unintended financial commitments without proper understanding or parental oversight. Additionally, the lack of transparency and explicit user consent in programs like [VOICE ASSISTANT FEATURE] raises concerns about involuntary data sharing and diminished user control over personal information.                                                                                                    & Users are concerned that they are automatically enrolled in free trials for subscription services without their explicit consent, resulting in the loss of key camera features once the trial expires. Additionally, they worry that vendors may access and share their footage with authorities without obtaining explicit consent or a warrant, raising serious privacy issues.                                                                                                                                                                                                                                                                                                            \\ \midrule
Data Accuracy                                    & Many reviewers report significant inaccuracies in fitness trackers' data, including step counts, calorie burn estimations, heart rate readings, and sleep tracking, with instances like blood pressure readings being markedly lower than calibrated measurements. This lack of data accuracy raises serious safety concerns, as users might unknowingly rely on faulty health metrics for important decisions, and coupled with invasive data collection practices, there's a risk that inaccurate health information could be collected and potentially misused. & Users have expressed concerns about [VOICE ASSISTANT]'s data accuracy due to its inability to accurately understand and process their spoken requests, resulting in frustration and potential privacy issues. An example highlights a user who reports that [VOICE ASSISTANT] frequently misinterprets basic American English, sometimes rendering their requests for classical music into offensive language.                                                                                                                                                & Users are reporting significant concerns about data accuracy, specifically pointing to unreliable motion detection that fails to capture important events like package thefts or break-ins while generating false alarms for minor movements such as passing cars or swaying branches. Additionally, inaccurate timestamps on recorded footage are making it difficult to determine the exact timing of events, potentially rendering the recordings useless for evidentiary purposes.                                                                                                                                                                                                       \\ \midrule
Data Collection                                  & Users are concerned that the fitness tracker and its app collect excessive personal information—such as location, contacts, call logs, and credit card details—which may be exploited for profit or surveillance. The lack of transparency about how this data is used and shared, particularly due to the app's connections with [FOREIGN COMPANIES], heightens distrust and anxiety over potential misuse of sensitive personal information.                                                                                                                       & Users are concerned that [VOICE ASSISTANT] devices are constantly listening and recording conversations without explicit activation, raising questions about the extent and purpose of [COMPANY]'s data collection. This data is potentially used for targeted advertising and personalized recommendations, leading to discomfort and feelings of being monitored among users who notice a direct correlation between their private conversations and subsequent ads.                                                                               & Users are expressing significant concerns about the extensive collection of personal data by home security camera systems, including phone numbers, email addresses, and biometric information. Many feel that this data collection exceeds what is necessary for the systems to function and are anxious about potential misuse by vendors, such as sharing data with third parties or law enforcement agencies.                                                                                                                                                                                                                                                                            \\ \midrule
Data Deletion                                    & Users are concerned that their data may not be fully deleted even after requesting account deletion or uninstalling apps, leaving sensitive information vulnerable to misuse. Additionally, accidental data loss due to software glitches or user errors, such as disappearing data or syncing issues, is a significant concern.                                                                                                                                                                                                                                   & Users face significant challenges when attempting to delete voice recordings and other data collected by [VOICE ASSISTANT] devices due to cumbersome processes and a lack of transparency. The absence of a simple option to delete all data at once raises concerns about the retention and potential misuse of sensitive personal information even after users try to delete it.                                                                                                                                                                & Users are concerned about their lack of control over data deletion, as many systems automatically purge recordings after a specific time period without user consent or the ability to extend retention, potentially leading to the loss of crucial evidence and raising privacy issues. Additionally, difficulties in managing local storage—such as the inability to bulk delete recordings and the need to physically remove storage devices—highlight the cumbersome and potentially insecure processes associated with data deletion.                                                                                                                                                   \\ \midrule
Data Exposure                                    & Users have expressed concerns about data exposure when purchasing [COMPANY] devices from unauthorized third-party resellers, fearing that these sellers might access their data or provide counterfeit devices with compromised security features. Additionally, there are worries about the app's invasive data collection practices and the company's potential sharing of user information with third parties, including data brokers.                                                                                                                             & Users are concerned that [COMPANY]'s requirement for mandatory account creation exposes their personal data to potential collection and sale to third parties. Additionally, there's apprehension that newer [BRAND] models, unlike the "[BRAND NAME]," monitor user data, possibly using it for monetization.                                                                                                                                                                                                                                        & Refurbished cameras that remain linked to previous owners' accounts can lead to data exposure, making personal information and sensitive recordings accessible to unauthorized individuals. Additionally, users are apprehensive about vendors collecting and sharing personal data through required phone number verification during setup, raising fears of data misuse and increased spam or targeted advertising.                                                                                                                                                                                                                                                                        \\ \midrule
Data Harms                                       & Users are reporting psychological harm due to inaccurate or potentially manipulated data from fitness trackers, such as concerns that health metrics are being inflated after a subscription lapse to encourage renewals. Additionally, reports of physical discomfort, including skin irritation and speculation about radiation exposure from the devices, highlight the need for greater transparency and safety in data handling and device usage.                                                                                                             & [VOICE ASSISTANT]'s misinterpretation of conversations and ambient noises can result in unintended actions, such as accidentally contacting emergency services, demonstrating the real-world data harms from inaccurate processing of user inputs. Additionally, there is concern over [VOICE ASSISTANT] manipulating or deceiving users through misleading marketing or unwanted subscriptions, particularly affecting vulnerable groups like children, which highlights potential abuses in data handling and user trust.                                   & Home security cameras pose significant data harms due to hacking and unauthorized access to camera feeds, resulting in harassment, privacy violations, and potential blackmail. Additionally, users are concerned that vendors may collect personal information and use it beyond security purposes, leading to data misuse and erosion of privacy.                                                                                                                                                                                                                                                                                                                                          \\ \midrule
Data Hiding                                      & -                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & The user's experience underscores how data hiding, such as concealing a Wi-Fi network's SSID, can lead to practical difficulties for legitimate users trying to connect smart devices like [COMPANY]'s [VOICE ASSISTANT]. While hiding a network is intended to enhance security by reducing visibility to unauthorized users, it can inadvertently complicate setup procedures and does not replace the need for robust security measures like strong encryption and passwords.                                                                     & Some users express a desire for features that allow them to better conceal security cameras and locally stored footage, emphasizing the importance of data hiding in their home security systems. One reviewer specifically wishes for a centralized storage solution that can be hidden in a secret corner, highlighting their need for greater control over the visibility and accessibility of their security data.                                                                                                                                                                                                                                                                       \\ \midrule
Data Management and Storage                      & Users are concerned about the security of personal data collected by fitness trackers, citing fears of unauthorized access or data breaches due to a lack of transparency in how the data is stored and managed. Additionally, issues like syncing problems, app malfunctions, and difficulties transferring data between devices raise concerns about the reliability of data storage and the potential for permanent data loss.                                                                                                                                  & Users are concerned about the centralized data storage within the [VOICE ASSISTANT] ecosystem, which diminishes their control over personal information. The daily transfer of security recordings from multiple devices to the cloud exacerbates worries about data security, privacy, and the risk of unauthorized access or misuse.                                                                                                                                                                                                            & Users are frustrated with confusing and restrictive local storage options, feeling misled into purchasing cloud subscriptions despite using SD cards or USB drives. Additionally, managing locally stored footage is slow and cumbersome, raising privacy concerns as it often requires manually deleting individual clips and physically removing storage devices.                                                                                                                                                                                                                                                                                                                          \\ \midrule
Data Security and Data Theft                     & Users are highly concerned about data security due to the app requiring storage of credit card information for "free" trials and subscriptions, leading to reports of unauthorized charges and account compromises. The absence of clear security measures and the app's connections to  [FOREIGN COMPANIES] further amplify fears of large-scale data breaches and the potential misuse of sensitive personal and health data.                                                                                                                                       & Users are concerned about data security and theft due to scammers exploiting the device setup process by impersonating Amazon technicians to gain remote access to their computers or obtain sensitive personal and financial information. Additionally, they fear that insufficient security and control within the [VOICE ASSISTANT] ecosystem could lead to unauthorized access, data breaches, and misuse of their personal data for purposes like targeted advertising.                                                                      & Users are concerned about data security vulnerabilities stemming from local storage on unencrypted SD cards, which are susceptible to theft and lack automatic backups. They also fear their data could be accessed or stolen through hacking and unauthorized account access, highlighting the need for stronger security measures.                                                                                                                                                                                                                                                                                                                                                         \\ \midrule
Data Sharing                                     & Users are concerned about the app's lack of transparency and control over their personal data, fearing it may be shared with third parties, sold to data brokers, or used for purposes beyond fitness tracking like targeted advertising or research. These worries are amplified by the app's connection to [FOREIGN COMPANIES], leading to unease about the potential sharing of their data with the [FOREIGN GOVERNMENT] or other entities.                                                                                                                         & Users are concerned about insufficient control over data sharing within the [VOICE ASSISTANT] ecosystem, particularly in multi-user households and with shared accounts, which leads to unintended access to personal information like shopping lists, purchase history, and connected devices. This lack of control results in unintended disclosures and privacy violations, including accidental sharing of data with external parties through voice messages or contact syncing.                                                              & Users are concerned that they cannot share access to their camera feeds with others without sharing login credentials, which poses security risks by granting full control over their systems. Additionally, they worry about vendors sharing their data with third parties, especially when camera systems are linked to accounts like [COMPANY], raising fears about data collection practices and potential misuse of personal information.                                                                                                                                                                                                                                                  \\ \midrule
General Comments Related to Security and Privacy & Users express widespread concerns about the security and privacy of fitness tracker apps, highlighting issues such as excessive personal data collection, lack of transparency in data usage, and the potential for data breaches or misuse of information. These fears are intensified by the apps' connections to companies in certain countries, leading to apprehension about data sharing with foreign governments, and are compounded by reports of phishing scams, unauthorized charges, and other malicious activities experienced after using the apps.   & Users of [VOICE ASSISTANT]-enabled devices grapple with the trade-off between convenience and privacy, acknowledging the risks of constant monitoring and data collection but often prioritizing functionality over privacy concerns. This tension highlights a societal trend of accepting privacy compromises for technological advancement, raising questions about data security and underscoring the need for greater transparency and control over personal data to alleviate anxieties about misuse or unauthorized access.                & Users often question the reliability and effectiveness of home security cameras due to technical issues like unreliable motion detection, delayed recording activation, short recording durations, and poor night vision, which can undermine their ability to deter crime or capture crucial evidence. Additionally, there are significant security and privacy concerns, as these systems may be vulnerable to hacking, data breaches, and unauthorized access to camera feeds and personal information.                                                                                                                                                                                   \\ \midrule
Location Tracking                                & Users are concerned that fitness tracker apps demand constant access to their location data, even when GPS features are not being used, fearing that their movements are being tracked and sensitive location information is being collected. This continuous location tracking, combined with vague privacy policies and connections to [FOREIGN COMPANIES], heightens anxieties about potential data misuse, surveillance, and the unauthorized sharing of location data with third parties.                                                                       & Users are concerned that devices require them to enable location services during setup, even when it's not essential for the device to function properly. This mandatory requirement, combined with a lack of transparency about how companies use their location data, raises fears of tracking, profiling, and targeted advertising without their informed consent.                                                                                                                                                                 & Users are expressing concerns about the accuracy of location tracking in security camera systems, where features can be improperly disabled because the system relies on IP address locations that may not reflect the actual physical location. There are also worries that the location data required during setup might be used beyond its intended purpose, potentially allowing vendors to collect data and track users without their consent.                                                                                                                                                                                                                                          \\ \midrule
Personalized Advertising                         & Users are frustrated with the fitness tracker app's aggressive personalized advertising, including frequent pop-up ads promoting additional products and services—even for those who have already purchased the device. This intrusive approach not only disrupts the user experience but also raises privacy concerns due to the potential reliance on extensive data collection and analysis for ad personalization.                                                                                                                                             & Many users are concerned that [VOICE ASSISTANT] devices are constantly listening to their conversations and using this information to deliver personalized advertising, as they often see ads related to topics they've only discussed verbally near the device. Additionally, there is frustration over [VOICE ASSISTANTS]'s unsolicited promotion of Amazon products and services, which can interrupt interactions with unexpected advertisements.                                                                                                          & Several reviewers are worried that vendors collect and use their personal data for personalized advertising without transparent consent, particularly due to the requirement to link their Amazon accounts for certain features. This lack of clarity in data collection and sharing practices leads to fears that companies like [COMPANY] are profiting from user data, with some users feeling manipulated into subscription services designed to maximize consumer dependency.                                                                                                                                                                                                              \\ \midrule
Policies and Law                                 & Users are concerned that [COMPANY]'s data collection practices and lack of transparency in its privacy policies may violate consumer protection laws by not providing adequate control over personal information. Additionally, the requirement to use proprietary charging cables and potential warranty issues could infringe upon consumer rights under applicable laws.                                                                                                                                                                                           & There are significant concerns that [COMPANY] may share user data with law enforcement agencies without requiring warrants or court orders, potentially eroding privacy rights and bypassing legal safeguards against government surveillance. Additionally, users are frustrated with [COMPANY]'s customer service practices, particularly regarding the handling of personal information and the potential for it to be exploited in scams.                                                                                               & Users are concerned that security camera footage could be accessed and shared with government agencies or law enforcement without consent or a warrant, highlighting potential violations of privacy laws and the misuse of personal information. They are also frustrated by the lack of transparency in vendor policies regarding data collection, storage, and sharing practices, which complicates their ability to understand and assert their rights under existing laws and regulations.                                                                                                                                                                                              \\ \midrule
Privacy Controls                                 & Users are frustrated by the lack of control over privacy settings, particularly the inability to customize notifications and limit data sharing with third parties. They express concerns about sensitive personal information being displayed without consent and the absence of parental controls to prevent children from receiving unwanted notifications.                                                                                                                                                                                                     & Users expressed significant privacy concerns about [DEVICES], particularly regarding the "always listening" feature and potential unauthorized access to their personal data. To address these issues, they attempted to use privacy controls such as unplugging the device when not in use, disabling certain features like [FEATURE], and deleting their recordings or activity history, although some found these controls difficult to navigate or insufficient.                                                         & Users are concerned about the lack of granular privacy controls in their systems, including the inability to customize notifications for specific individuals or events, limited control over motion detection zones and sensitivity, and restricted options for privacy modes and scheduling—resulting in excessive notifications, inaccurate motion detection, and a constant feeling of being monitored. Additionally, they express frustration over limited control of data sharing and access, worried that vendors may share sensitive personal information with third parties or authorities without explicit consent, raising ethical concerns about potential misuse of their data. \\ \midrule
Privacy Ethics                                   & Users express privacy ethics concerns regarding [COMPANY]'s use of manipulative design tactics, such as requiring excessive permissions and persistently pressuring them to provide credit card information despite prior refusals. Additionally, there is unease about the potential misuse of sensitive health data for marketing or profit-driven purposes, which may compromise user privacy.                                                                                                                                                                     & Many users are ethically concerned that [COMPANY]'s data collection practices violate their privacy by constantly recording and potentially sharing personal conversations without clear consent. The lack of transparency about what data is collected, how it's used, and who has access to it amplifies these concerns, suggesting that [COMPANY] prioritizes profit over user privacy.                                                                                                                                                  & Users are troubled by security cameras that continue to operate even when they believe the devices are off, leading to feelings of discomfort and a violation of privacy within their own homes. This situation raises ethical concerns about the balance between security and privacy, emphasizing the need for stronger privacy controls to prevent unauthorized recording and misuse of sensitive footage in home security systems.                                                                                                                                                                                                                                                       \\ \midrule
Secure Communication                             & Users are concerned that the device's always-on Bluetooth requirement for syncing and accessing features could pose security risks in terms of secure communication. They fear that this continuous connection may expose their personal data to unauthorized access or interception, especially given anxieties about the app's data collection practices and its connections to [FOREIGN COMPANIES].                                                                                                                                                               & Users are facing challenges connecting to secure Wi-Fi networks that use hidden SSIDs or long, complex passwords, which may prompt them to weaken their security by opting for less secure networks or by revealing their network names. Similarly, concerns about unauthorized Bluetooth connections arise because devices often automatically connect or broadcast their availability, potentially exposing personal information and compromising secure communication.                                                             & Users are concerned that the reliance on an active internet connection for many camera systems, even when using local storage, poses risks of service disruptions and potential data breaches during internet outages or malicious attacks. They also worry about the lack of transparency in data transmission, fearing that recordings might be sent to the cloud before being stored locally, which could allow unauthorized access during these transfers.                                                                                                                                                                                                                               \\ \midrule
Security Vulnerabilities                         & Users are concerned that fitness trackers and their associated apps may have security vulnerabilities that could be exploited by hackers and malware, potentially leading to data theft, financial fraud, and device malfunctions. Reports of suspicious activities such as browser lag, app freezing, unauthorized access to connected devices like [VOICE ASSISTANT], and fraudulent transactions have heightened anxieties about the security of these devices and the potential for exploitation by malicious actors.                                                      & Users are experiencing security vulnerabilities where devices are being hacked or accessed without authorization, leading to incidents like strangers' voices coming through speakers and devices connecting to personal accounts without permission. These breaches also include devices randomly calling contacts, which amplifies concerns about the ease of unauthorized access and control over personal devices and data.                                                                                                       & Home security cameras are facing significant security vulnerabilities due to physical insecurity, as users report that these devices can be easily detached from their mounts or have their batteries stolen, compromising their effectiveness. Additionally, there are numerous reports of systems being hacked, allowing unauthorized individuals to access camera feeds, manipulate settings, and even communicate through the cameras, which severely undermines the intended security purpose of these devices.                                                                                                                                                                         \\ \midrule
Software and Firmware Updates                    & Users are concerned that software and firmware updates may introduce new security vulnerabilities or worsen existing ones, with incidents like devices becoming "bricked" during updates highlighting these risks. Additionally, frequent and intrusive update requests without clear information about their purpose and content have led to user frustration.                                                                                                                                                                                                    & Forced software and firmware updates can introduce new bugs or vulnerabilities, disrupt device functionality, and compel users to accept updates to continue using their devices. The lack of transparency about the content and purpose of these updates heightens concerns about potential security risks and data collection practices.                                                                                                                                                                                            & Users are concerned that mandatory firmware updates disable previously free features, forcing them to subscribe to paid services to regain functionality. Additionally, these updates often introduce bugs, glitches, and connectivity issues, undermining the reliability and security of their camera systems.                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
Surveillance                                     & Users are concerned that the app's extensive collection of personal data—such as sleep patterns, location, and heart rate—could lead to surveillance or misuse by third parties without their consent. Specifically, worries about the app's connections to [FOREIGN COMPANIES] raise fears that data might be shared with the [FOREIGN GOVERNMENT] or other entities for surveillance or malicious purposes.                                                                                                                                                          & Users are highly anxious about the "always-on" nature of smart speakers, fearing they enable constant surveillance by continuously recording conversations and sharing data with [COMPANY], the government, or other third parties. Unexpected activations without a clear "wake word" and responses to unintended cues amplify these concerns, reinforcing the perception that the devices are "spying" on them.                                                                                                                        & Users are concerned that security cameras can be used for unwanted or unauthorized surveillance, fearing that strangers, landlords, or even family members might access the cameras without their knowledge or consent. They also express worries about the limited control over the cameras' surveillance capabilities—such as adjusting motion detection sensitivity or disabling recording—which leads to feelings of constant monitoring and a loss of privacy within their own homes.                                                                                                                                                                                                   \\ \midrule
Trust and Transparency                           & Many users feel misled by [COMPANY] because of ambiguous marketing around subscription requirements and the true costs of accessing the device's full functionality. This lack of transparency, combined with frequent updates that change app features, has eroded trust and made it challenging for users to assess the security and privacy implications of using the device.                                                                                                                                                                                      & Users distrust [COMPANY]'s data practices due to concerns about undisclosed data sharing and forced enrollment in programs like [FEATURE] that share user bandwidth. This lack of transparency in data collection and usage, combined with aggressive upselling tactics and potentially deceptive marketing, leads to feelings that [COMPANY] prioritizes profit over user privacy and well-being.                                                                                                                                           & There is a significant erosion of trust between customers and security camera vendors due to a lack of transparency, with many users feeling misled by unclear product descriptions, hidden subscription requirements, and limitations on local storage that were not disclosed upfront. Additionally, concerns over data collection practices, such as sharing user data with third parties and potential access by authorities, further diminish trust as customers discover these issues only after purchase.                                                                                                                                                                             \\ \midrule
Usability                                        & Constant requests for sensitive information like credit card details and location access, combined with unclear instructions and complex navigation, lead users to view these usability issues as intrusive attempts to access their data. This poor usability undermines trust, making it difficult for users to understand and manage privacy settings and data sharing options.                                                                                                                                                                                 & Users find it challenging to manage their privacy with smart speakers due to always-on microphones and data collection practices that are not user-friendly. Issues like difficulty deleting recordings, unexpected activations, and unclear data usage policies create usability problems that affect their ability to control personal information.                                                                                                                                                                                 & A significant usability issue highlighted is the slow and laggy performance of the apps and cameras, which leads to missed events, delayed notifications, and difficulty accessing live feeds. Furthermore, the lack of user-friendliness in the apps and system interfaces—evident in poor documentation, confusing setup processes, and limited control over camera settings—poses additional challenges for users.                                                                                                                                                                                                                                                                        \\ 
\bottomrule
\end{xltabular}

==> Table/p_ft.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\resizebox{0.5\textwidth}{!}{\begin{tabular}{@{}llr@{}}
\toprule
\textbf{ASIN} & \textbf{Product}                  & \multicolumn{1}{l}{\textbf{No. of Reviews}} \\ \midrule
B09BXQ4HMB    & Fitbit Charge 5                   & 4783                                        \\
B08DFGPTSK    & Fitbit Inspire 2                  & 4760                                        \\
B08DKYLK4D    & Amazfit Band 5                    & 4670                                        \\
B08XM8X4VQ    & KALINCO Smart Watch               & 3118                                        \\
B09LMD1WL4    & Kummel Fitness Tracker            & 1075                                        \\
B08PF9V27X    & ENGERWALL Fitness Tracker         & 896                                         \\
B0B5FGP237    & Fitbit Inspire 3                  & 809                                         \\
B09PRHRTKG    & Pautios Smart Watch               & 802                                         \\
B0BCWQ6P99    & KAKTIN Smart Watch                & 609                                         \\
B0BVLVBYPJ    & Smart Watch Fitness Tracker       & 470                                         \\
B09M3LQ6WB    & threesheep Fitness Tracker        & 444                                         \\
B09QBVD7BY    & aeac Smart Watch                  & 411                                         \\
B0BLYV4B1L    & DoSmarter Fitness Tracker         & 297                                         \\
B0C1N9VDMM    & Ddidbi Smart Watch                & 199                                         \\
B0BTBX691N    & Fitness Tracker(Answer/Make Call) & 175                                         \\
B0BY89CPDQ    & ASWEE Smart Watch                 & 169                                         \\
B0BW43XJ94    & TOOBUR Smart Watch                & 141                                         \\
B0BR9TBF8Q    & WalkerFit A1 Smart Watch          & 130                                         \\
B0BTPHY136    & Fitness Tracker                   & 44                                          \\
B0BTZ4SN9S    & Fitness Tracker                   & 24                                          \\
B0C3XWPM18    & Fitness Tracker                   & 18                                          \\
B09BXH5MC1    & Fitbit Charge 5                   & 1                                           \\
B0BVLWKNKR    & Smart Watch Fitness Tracker       & 1                                           \\ \bottomrule
\end{tabular}}
\end{table}

==> Table/p_shs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{@{}llr@{}}
\toprule
\textbf{ASIN}       & \textbf{Product}                        & \multicolumn{1}{l}{\textbf{No. of Reviews}} \\ \midrule
B06XXM5BPP & Echo (2nd Gen)                 & 4911                               \\
B07G9Y3ZMC & Echo Studio                    & 4516                               \\
B07XKF5RM3 & Echo (4th Gen)                 & 4354                               \\
B07XJ8C8F5 & Echo Dot (4th Gen)             & 4323                               \\
B07FZ8S74R & Echo Dot (3rd Gen)             & 4140                               \\
B07F2H1LHL & XLeader SoundAngel A8          & 2424                               \\
B09B8W5FW7 & Echo Dot (5th Gen)             & 1495                               \\
B07NJPXRBC & Sonos One (Gen 2)              & 1038                               \\
B07W6RYRZM & Sonos One SL                   & 880                                \\
B07FDF9B46 & Bose Home Speaker 500          & 873                                \\
B08MQYNHWD & Sonos Move                     & 814                                \\
B08VKXP1VY & Bose SoundLink Revolve II      & 591                                \\
B09QC4X5S4 & SEREONIC TV Speakers           & 419                                \\
B084KYM1HH & Refurbished Echo Dot (4th Gen) & 373                                \\
B07NQD5L6V & Refurbished Echo Studio        & 362                                \\
B085PNV4SK & Refurbished Echo (4th Gen)     & 229                                \\
B08HPXPTSB & Belkin SOUNDFORM Elite         & 145                                \\
B07PN63DCP & Sonos One (Gen 2)              & 75                                 \\
B077GK3TTQ & Sonos Two Room Set             & 68                                 \\
B09SJ4RL8M & Precision Pro Ace GPS Speaker  & 52                                 \\
B09Q82T1ZL & BESTISAN 100W Subwoofer        & 38                                 \\
B09R4ZF2QW & Turtlebox Gen 2                & 27                                 \\
B09R4XLCV3 & Turtlebox Gen 2                & 18                                 \\
B09R4YXC7W & Turtlebox Gen 2                & 14                                 \\ \bottomrule
\end{tabular}}
\end{table}

==> Table/p_sscs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{@{}llr@{}}
\toprule
\textbf{ASIN} & \textbf{Product}                  & \multicolumn{1}{l}{\textbf{No. of Reviews}} \\ \midrule
B086DKMSSM    & Blink Outdoor (3rd Gen)           & 4719                                        \\
B07X6C9RMF    & Blink Mini Indoor Camera          & 4537                                        \\
B0758L64L9    & Ring Spotlight Cam                & 4097                                        \\
B08B3B3LQ3    & Arlo Spotlight Camera             & 3905                                        \\
B0B5GRGB58    & Wireless Outdoor Cameras          & 3385                                        \\
B08GHX9G5L    & Kasa Pan/Tilt Camera              & 2762                                        \\
B07X5FCW3X    & Blink Indoor (3rd Gen)            & 2036                                        \\
B0BD5VXKGW    & Galayou 2K Indoor Camera          & 1512                                        \\
B0866S3D82    & TP-Link Tapo Indoor Camera        & 1424                                        \\
B0BJ6XQ78R    & Wireless Cameras                  & 1341                                        \\
B00L3W2QJ2    & ANNKE 3K Camera System            & 724                                         \\
B09HC4ZJBL    & LaView 4MP Cameras                & 719                                         \\
B0BKG4Z1NK    & IHOXTX Cameras                    & 691                                         \\
B016UCNP3A    & REOLINK 5MP Camera System         & 605                                         \\
B09P33NVRF    & 2K (3MP) Cameras                  & 504                                         \\
B09Q38Y8NH    & Acelerar 2K Outdoor Camera        & 474                                         \\
B00NBT224O    & ZOSI 1080p Camera System          & 430                                         \\
B09J6Y8Y73    & Nest Indoor Cam                   & 304                                         \\
B0BJBH3XGZ    & Tashi Light Bulb Camera           & 284                                         \\
B08WFJKK2T    & Arlo Indoor Camera                & 253                                         \\
B082KGF6FX    & REOLINK 4K Camera System          & 231                                         \\
B0B5VLCL1N    & Blink Floodlight Camera           & 215                                         \\
B0BX9ZKQKT    & Outdoor Wireless Cameras          & 148                                         \\
B0816DWCD5    & Hiseeu 5MP Wired Camera System    & 122                                         \\
B0BX3MJHN6    & Gerdviaw 2K Cameras               & 88                                          \\
B0BMKK2SX5    & Camland Solar Camera System       & 10                                          \\
B086DKSHQ4    & Blink Outdoor (3rd Gen)           & 2                                           \\
B08PBR83NM    & Blink Mini Indoor Camera (3-Pack) & 2                                           \\ \bottomrule
\end{tabular}}
\end{table}

==> Table/related-work-tabel.tex <==

\begin{table*}[!t]
\caption{Comparison of NLP-based analysis of user comments or reviews in prior works versus our study.}
\begin{tabularx}{\textwidth}{@{} l p{4cm} X p{2.75cm} X X p{1.25cm} @{}}
\toprule
\textbf{Reference} & \textbf{Task}                                         & \textbf{Text}       & \textbf{Model used}                       & \textbf{Taxonomy used}        & \textbf{Prompt Engineering} & \textbf{Rating analysis} \\ \midrule
\multirow{2}{*}{Henao et al. \cite{henao2021transfer}}      & Mining feature requests and bug reports               & User comments       & BERT (Monolingual + Bilingual)            & No                              & No                          & No                       \\ \midrule
\multirow{2}{*}{Palomba et al. \cite{palomba2017recommending}}     & Recommending and localizing change requests           & App reviews         & Classical NLP (Text + Sentiment analysis) & No                              & No                          & No                       \\ \midrule
\multirow{2}{*}{Fu et al. \cite{fu2013people}}          & Users' likes and dislikes towards apps                & App reviews         & LDA                                       & No                              & No                          & Yes                      \\ \midrule
\multirow{2}{*}{de Ara\'ujo et al. \cite{de2021re}} & Identification of software requirements               & App reviews         & BERT                                      & No                              & No                          & No                       \\ \midrule
\multirow{2}{*}{Harkous et al.\cite{harkous2022hark}}     & Eliciting privacy concerns                            & App reviews         & T5 with hypothesis based NLI technique    & Privacy              & No                          & No                       \\ \midrule
\multirow{2}{*}{Akgul et al. \cite{akgul2024decade}}       & Analyzing decade-long privacy concerns in app reviews & App reviews         & T5 architecture with static prompt        & Privacy              & Yes (static)                & No                     \\ \midrule
\multirow{2}{*}{Our work}           & Mining S\&P concerns in IoT product reviews             & IoT product reviews & GPT-3.5-turbo                             & S\&P  & Yes (dynamic)               & Yes                      \\ \bottomrule
\end{tabularx}
\vspace{-12pt}
\end{table*}

==> Table/review-crc-tm.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!t]
\fontsize{2.8mm}{2.8mm}\selectfont
\caption{At the left, there are three reviews from the test dataset. In the middle, there are Task 3 responses from the CRC model for these reviews (Notice that Task 3 responses are non-null only if Task 1 response is a ``Yes"). At the right, there are mappings from the TM model for each low-level theme.}
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabularx}{\textwidth}
{ X| >{\hsize=.7\hsize}X| X} 

% \begin{tabularx}{XXX} 

\toprule
\textbf{Review}                                                                                                                                                                                                                                                                                                                                                                                                             & \textbf{CRC's Task 3 Response}                                                                                                                                                & \textbf{TM's low-level to high-level mapping}                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
SSCS-3132: \textit{I bought this with no intention of utilizing the subscription and doing only local storage. ... (gap) ... the subscription paywall as well. Now I can only use them as live feed as any other service is blocked without paying them extra. Only buy Blink if you’re planning to buy the subscription as well} & Task 3: concerns about the subscription model, limited access to security features, potential data collection and privacy implications                                          & \begin{itemize}
    \item concerns about the subscription model -\textgreater business practice transparency,\item limited access to security features -\textgreater access control, usability, user preference,\newline potential \item data collection and privacy implications -\textgreater data collection, privacy invasion                                                          \end{itemize}                                                                               \\ \midrule
SHS-3648: \textit{It evesdrops on my conversations and allows amazon and whomever has money to listen in. ... (gap) ...}                                                                                                                                                                                                                                                                    & Task 3: concerns about eavesdropping, concerns about unauthorized listening, concerns about the device being always on, surveillance, lack of control over personal information & \begin{itemize} \item concerns about eavesdropping -\textgreater eavesdropping, surveillance, privacy invasion, \item concerns about unauthorized listening -\textgreater eavesdropping, surveillance, intrusion, \item concerns about the device being always on -\textgreater privacy invasion, surveillance, seclusion, \item surveillance -\textgreater surveillance , \item lack of control over personal information -\textgreater privacy controls \end{itemize}                                                   \\ \midrule
FT-26162: \textit{... (gap) ... The app was created in, and comes from China. Wanted a lot of permissions. ... (gap) ... I just didn't like it and didn't want to use the China app. Returned.}                                                               & Task 3: app permissions, data privacy, trustworthiness of the app, country of origin of the app                                                                                 & \begin{itemize}
    \item app permissions -\textgreater consent, system/application, technical and technological issues, \item data privacy -\textgreater data privacy, \item trustworthiness of the app -\textgreater trust, system/application , \item country of origin of the app -\textgreater affiliation with a country or a geographic region \end{itemize}                                                                                             \\ \bottomrule
\end{tabularx}
\label{revcrctm}
}
\end{table*}

==> Table/topics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[!t]
\caption{Partition of the 85 high-level themes to relevant topics.}
\centering
\resizebox{0.9\textwidth}{!}{\begin{tabularx}{\textwidth}{>{\hsize=.4\hsize\linewidth=\hsize}X |
>{\hsize=1.6\hsize\linewidth=\hsize}X}
\toprule
\textbf{Topic}                   & \textbf{High-level Themes}                                                                                                                                                                                                                                                                                                     \\ \midrule
Data Security                    & access control, authentication, authorization, data availability, data confidentiality, data deletion, data exposure, data integrity, data modification, data security, encryption and confidentiality, identification, password issues, payment security, secure communication, software and firmware updates \\ \midrule
Trust and Transparency           & business practice transparency, company's affiliation, lack of trust in the device, notice / awareness, transparency, trust, privacy invasion                                                                                                                                                                                                              \\ \midrule
Security Threats and Incidents   & appropriation, breach of confidentiality, blackmail, concerns or vignettes about hackers, device hacking, eavesdropping, fraud, intrusion, invasive customer support, lack of authentication and authorization, malware, software/hardware bugs                                                                                \\ \midrule
Privacy Controls and Preferences & access / participation, choice / consent, consent, data minimization, data privacy, privacy controls, privacy preservation, purpose specification, remove personally identifiable information, responsiveness, seclusion, unlinkability, use limitation, user preference                                                       \\ \midrule
Monitoring                       & location and tracking, surveillance, tracking                                                                                                                                                                                                                                                                                  \\ \midrule
Physical and System Security     & intrusion detection, issues with apps, physical security, safety, system/application, technical and technological issues, wi-fi security                                                                                                                                                                                                      \\ \midrule

User Interaction and Usability   & ease of adoption, usability                                                                                                                                                                                                                                                                                                    \\ \midrule
Data Handling and Processing     & advertising, data collection, data disclosure, data misuse, data sharing, information dissemination, information processing, onward transfer, selling data, storage                                                                                                                                                            \\ \midrule
General Concerns                 & being self-righteous about privacy, generic privacy issues, generic security issues, humor or sarcasm to express concerns, insecurity, personal skepticism and opinions, recognizing privacy concerns but showing indifference, trading privacy for utility                                       \\ \midrule
Legal and Ethical Considerations & affiliation with a country or a geographic region, government oversight, privacy policies and laws, surveillance by a government or a regime                                                                                                                                                                                   \\ \midrule

Fairness and Ethical Use         & fairness, decisional interference                                                                                                                                                                                                                                                                                              \\ \bottomrule
\end{tabularx}\label{elevenbroadtopics}}
\end{table*}

==> Table/ttest.tex <==
\begin{table}[!t]
\centering
\caption{2-sample $t$ test. $H_{0}:$ $\mu_{c} = \mu_{n}$, vs. $H_{A}:$ $\mu_{c} < \mu_{n}$. $\bar{y}_{c}$ and $\bar{y}_{n}$ are the sample average ratings of the concern and non-concern reviews, respectively. The significance code *** means $p < .001$.}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\textbf{Device} & \multirow{2}{*}{\textbf{$\bar{y}_{c}$}}    & \multirow{2}{*}{\textbf{$\bar{y}_{n}$}}     & \multirow{2}{*}{\textbf{$t$}} & \multirow{2}{*}{\textbf{$df$}} & \multirow{2}{*}{$p-value$} \\
\textbf{type} &  &  & &  & \\ 
\midrule
FT                   & 2.35 ($n$ = 505 ) & 3.54 ($n$ =  23389) & -17.322     & 528.05         & $\textless 2.2e-16$***        \\
SHS                  & 3.88 ($n$ = 847) & 4.31 ($n$ = 31222) & -9.1732    & 878.8      &  $\textless 2.2e-16$***          \\
SSCS                 & 3.08 ($n$ = 3544) & 4.00 ($n$ = 31642)  & -32.306    & 4193.3      &  $\textless 2.2e-16$***        \\ 
Overall                 & 3.14 ($n$ = 4896) & 3..98 ($n$ = 86253)  & -35.642    & 5328.7      &  $\textless 2.2e-16$***        \\ 
\bottomrule
\end{tabular}}
\label{2samplettest}

\end{table}
